LMGP: Lifted Multicut Meets Geometry Projections for Multi-Camera Multi-Object Tracking

Multi-Camera Multi-Object Tracking is currently drawing attention in the computer vision field due to its superior performance in real-world applications such as video surveillance in crowded scenes or in wide spaces. In this work, we propose a mathematically elegant multi-camera multiple object tracking approach based on a spatial-temporal lifted multicut formulation. Our model utilizes state-of-the-art tracklets produced by single-camera trackers as proposals. As these tracklets may contain ID-Switch errors, we refine them through a novel pre-clustering obtained from 3D geometry projections. As a result, we derive a better tracking graph without ID switches and more precise affinity costs for the data association phase. Tracklets are then matched to multi-camera trajectories by solving a global lifted multicut formulation that incorporates short and long-range temporal interactions on tracklets located in the same camera as well as inter-camera ones. Experimental results on the WildTrack dataset yield near-perfect performance, outperforming state-of-the-art trackers on Campus while being on par on the PETS-09 dataset.

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/abstract.tex <==
\begin{abstract}
Multi-Camera Multi-Object Tracking is currently drawing attention in the computer vision field due to its superior performance in real-world applications such as video surveillance with crowded scenes or in wide spaces. In this work, we propose a mathematically elegant multi-camera multiple object tracking approach based on a spatial-temporal lifted multicut formulation. Our model utilizes state-of-the-art tracklets produced by single-camera trackers as proposals. As these tracklets may contain ID-Switch errors, we refine them through a novel pre-clustering obtained from 3D geometry projections.  As a result, we derive a better tracking graph without ID switches and more precise affinity costs for the data association phase. Tracklets are then matched to multi-camera trajectories by solving a global lifted multicut formulation that incorporates short and long-range temporal interactions on tracklets located in the same camera as well as inter-camera ones. Experimental results on the WildTrack dataset yield near-perfect performance, outperforming state-of-the-art trackers on Campus while being on par on the PETS-09 dataset. We will release our implementations at this link  \href{https://github.com/nhmduy/LMGP}{https://github.com/nhmduy/LMGP}.
% We will make our implementations available upon acceptance of the paper \footnote{ \href{https://github.com/nhmduy/LMGP}{https://github.com/nhmduy/LMGP}.}.


%In contrast to prior works, we refine these initial tracklets, which possibly contain ID-Switch errors, through a novel pre-clustering \textcolor{red}{obtained from} 3D geometry projections. As a result, we obtain better tracking graphs without ID switches and more precise affinity costs for the data association phase. Tracklets are then matched \roberto{to} multi-camera trajectories by solving a global lifted multicut 
%formulation over a tracking graph that incorporates short and long-range temporal interactions \textcolor{red}{on tracklets located in the same camera} as well as inter-camera ones. Experimental results on the WildTrack dataset yield near-perfect result, outperforming state-of-the-art trackers in Campus while being on par on the PETS-09 dataset. Our implementation \textcolor{red}{will be made available upon acceptance of the paper}.
\end{abstract}



==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/acknowledgment.tex <==
\vspace{-0.1in}
\section{Acknowledgements}
% This research is completed through the sponsor of BMBF under the project XAINES (grant no. 01IW20005).
This research is sponsored by the XAINES and pAItient projects (BMBF grant no. 01IW20005 and BMG grant no. 2520DAT0P2 respectively).

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}
% We have showed that a single optimization model and the use of 3D geometry can deliver almost optimal results in crowded scenes given good enough data, together with a the combination of powerful appearance features and state-of-the-art tracklet proposals. % and the use of 3D geometry in a
%
% We have shown that the combination of state-of-the-art tracklet proposals and the 3D geometry in a single optimization model can deliver almost optimal results in crowded scenes given good enough input data. 
We have shown that integrating single view-based approaches and centralized representation-based methods for multi-camera tracking can lead to improvements w.r.t.\ strategies that fall into only one of these paradigms. Given a good enough input data, this strategy can deliver almost optimal results even in crowded scenes.
We conjecture that in noisier settings, significantly better results can be achieved by making our 3D pre-clustering more robust, e.g., by employing it in an end-to-end training framework \citep{xu2020train,braso2020learning}.

%Our spatial-temporal global optimization model utlizing state of the art single camera trackers and powerful 3D-based affinities can improve significantly upon state of the art in multi-camera tracking.
%However, large improvements are dependent upon precise detections and objects that are not too far from the camera.
%We believe that further improvements can be obtained by making our clustering step more robust for noisy and small detections.
%We have proposed a spatial-temporal global optimization model utilizing state of the art single camera trackers and powerful 3D-based affinities as well as 3D-based tracklet preprocessing.
%We have shown that under the right conditions, i.e.\ good bounding boxes and enough cameras covering a scene calibrated well enough as in the WildTrack dataset, near perfect tracking results can be achieved even in crowded scenes with many occlusions.
%Additionally, we can achieve state-of-the-art results in the Campus dataset where bounding boxes are poorer. Finally, since we use single-camera tracker for tracklet proposals and lifted multicut solvers for global tracklet association, our approach will benefit from advances in these components which is contrast to approaches that use ad-hoc methods \cite{fleuret2007multicamera,you2020real}. 

% Currently, our pre-clustering method for grouping detections across cameras is sensitive to poor bounding boxes and mis-calibrated cameras. A more robust clustering step that would improve our performance in noisy settings is one of our future work.



==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/discussion.tex <==
\section{Discussion}
Besides a novel spatial-temporal lifted multi-cut formulation, our essential contribution is the 3D-based pre-clustering; thereby, we could address both perturbations in tracking graphs and composing high-quality affinity costs. Due to the 3D constraints assumption, this clustering step will depend on how calibrated camera parameters and bounding boxes are correct. While the camera parameters are simple to control, the bounding boxes are much more challenging as they are influenced by detectors and camera poses.  In our experiments, WILDTRACK satisfies these requirements, while in PETS-09, the bounding boxes are inferior due to the camera's position, and the DPM detector was employed. Consequently, we could achieve state-of-the-art performance on WILDTRACK with a large margin while much lower in PETS-09. In short, this phenomenon gives an insight idea that our method is highly suitable to track over a medium space given good detectors with multi-camera. We thus consider the obstacles to track in a vast space as challenges for future works. 
% For instance, if the camera positions are too far away targets tracking , even a state-of-the-art detector may suffer with small and error bounding boxes. Similarly, if the camera pose is close enough to pedestrian objects, low quality bounding boxes by a detector still may occur.

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/experiments.tex <==
\section{Experimental Analysis}
Below we detail our experimental setup and results, including implementation details of our approach, considered datasets and baselines, quality metrics, and ablations.
%We first detail the pre-clustering accuracy as this component has a large impact on graph quality and accuracy of affinity costs (Table~\ref{tab:temporal-costs-performance}, \ref{tab:spatial-costs-performance} and~\ref{tab:center-tracktor} Appendix). We then compare LMGP with current modern multi-camera methods on three datasets and show state-of-the-art performance.
%Ablation studies are also presented to better understand the behavior of our model.
%Finally, we illustrate the benefit of our lifted formulation through jointly reasoning on both spatial-temporal edges by comparing with a two-step strategy, i.e.\ optimizing on each view independently and then linking results in the next step. 


% We first detail pre-clustering performance and the global tracking graph pre-processing procedure.
% These components of our pipeline have a large impact on the final tracking outcome. 
% We then compare with current modern multi-camera methods on two datasets and show state-of-the-art performance.
% Along with it, ablation studies are also presented to better understand the behavior of our model.
% Finally, we illustrate how much multi-camera can improve against single-camera pedestrian tracking in crowded scenes.

\subsection{Implemention Details}

\myparagraph{Tracking Graph}
% , a recent state-of-the-art single-camera tracker, 
We use CenterTrack~\cite{zhou2020tracking}, one of current state-of-the-art single-camera trackers, to create tracklets for each camera.
These tracklets will be aligned again with the provided public detections to eliminate duplicated ones and retain detections that were not tracked, e.g.\ due to occlusion.
We apply DG-Net~\cite{zheng2019joint} for extracting embedding vectors for detections and train it on visible detections (Eq.~\ref{eq:occlusion-filtering}) obtained by running the proposed pre-clustering algorithm over training video sequences.
Finally, we train three basic multi-layer deep networks for the three networks $f_{\mathrm{split}}$, $f_{\mathrm{spatial}}$, and $f_{\mathrm{temporal}}$ which handle splitting up initial tracklets, generating affinity costs for spatial and temporal edges respectively.

\myparagraph{Lifted Multicut Solver}
For solving the proposed lifted multicut problem (Eq. \ref{eq:proposed-lmp}), we use the efficient GAEC+KLj heuristic solver from~\cite{keuper2015lifted}.
We adapt a two-stage optimization approach. First, the initial tracklets are used as nodes in the tracking graph and compute trajectories through the lifted multicut.
Second, we initialize the computed trajectories again as nodes in the tracking graph and recompute costs to obtain the final trajectories. The second step improves the trajectories computed in the first pass by allowing to compute costs on longer trajectories and joining trajectories together where a connection was not initially detected. For a long-time video, this process can be iterated until converged. More details of our implementations are described in Subsection \ref{sec:implement} Appendix.
% We give running times for the solver in Table~\ref{tab:running-time} Appendix.
% Our solver processes on average $1.9$ fps for the largest sequence. 

\subsection{Datasets \& Metrics}
We perform experiments on three datasets with a wide range of different camera configurations, densities, and video/bounding box qualities.
For all datasets, we use the provided detections for a fair comparison.% and validate performance on standard metrics from MOTChallenge~\cite{leal2015motchallenge,milan2016mot16}.

\begin{packed_description}
\item[- \normalfont\textit{WILDTRACK}~\cite{chavdarova2018wildtrack}:]
The largest-scale dataset for the multi-camera setting is currently with a dense group of $313$ pedestrians standing and walking.
There is a total of $400$ frames observed from seven cameras that are annotated with 3D positions.
The first $360$ of those frames is used for training and the rest for testing. 
\item[- \normalfont\textit{Campus}~\cite{xu2016multi}:] We have chosen the two sequences \textit{Garden~1} and \textit{Parking~Lot} which had camera calibration parameters and a ground plane for 3D-projection. There are 15 - 25 pedestrians in each video observed by four cameras captured at a 30fps rate.
For each video, we use the first $10\%$ for training and the remaining frames for testing. 
\item[- \normalfont\textit{PETS-09}~\cite{ellis2009pets2009}:]
Contains three sequences with increasing level of difficulty:
low density (S2.L1) - $19$ objects in $795$ frames, medium density (S2.L2) - $43$ pedestrians spreading in $436$ frames and high density (S2.L3) - $44$ pedestrians moving together in $240$ frames.
While PETS-09 is not as dense as WILDTRACK, its main challenge lies in its poor video acquisition conditions with cameras far away from targets and low-quality bounding boxes. 
\end{packed_description}
\vspace{-0.1in}
We report results for the following metrics:
\begin{packed_description}
\item[- \normalfont MOTA~\cite{bernardin2008evaluating}:] the multiple objects tracking accuracy measuring a number of false negatives (FN), false positives (FP), and identity switches (IDs) focusing on the coverage of detections. 
\item[- \normalfont MOTP~\cite{bernardin2008evaluating}:]
the multiple object tracking precision penalizes the overall dissimilarity between true positives and the ground truth objects.
\item[- \normalfont IDF1~\cite{ristani2014tracking}:] 
measure through the F1 score agreement between computed and ground truth trajectories.
%
%Based on a matching between computed trajectories and ground truth trajectories, the IDF1 score is the F1 score between the proportion of detections from computed trajectories that are matched to detections from ground-truth trajectories and ground truth detections that are  matched to detections from computed trajectories. 
%
%The F1 score between the relative number of computed detections matched ground truth trajectories and the relative number of ground truth detections matched to computed trajectories.
%
%proportion of correctly identified detections over the average number of ground-truth and computed detections.
\item[- \normalfont MT \cite{li2009learning}:] number of mostly tracked objects for at least $80\%$ of its life span.
\item[- \normalfont ML \cite{li2009learning}:] number of mostly lost objects for at most $20\%$ of its life span.
%\item[- \normalfont IDs \cite{bernardin2008evaluating}:] number of erroneous ID-switches.
\end{packed_description}
\subsection{Algorithms}
We compare against state-of-the-art baselines for each respective dataset.
To study the effectiveness of our approach and judge the effectiveness of each proposed component, we run experiments on multiple configurations. All algorithms are listed below.
\begin{packed_description}
\item[\normalfont\texttt{Baselines}:]
For each dataset, we compare against the most recent approaches for which we found experimental results.
In particular, we compare against KPS-DO,  KSP-DO-ptrack  \citep{chavdarova2018wildtrack}, GLMB-YOLOv3, GLMB-DO  \citep{9242263}, DMCT, DMCT Stack \cite{you2020real}, HJMV~\cite{hofmann2013hypergraphs}, STVH~\cite{wen2017multi}, MLMRF~\cite{lan2020semi}, HCT~\cite{xu2016multi}, STP~\cite{xu2017cross}, TRACTA~\cite{he2020multi} and DyGLIP~\cite{quach2021dyglip}.
All baseline performances are taken from the respective original papers. 
\item[\normalfont Our configurations are:]
\item[\normalfont\texttt{- LMGP w/o Pre-Clustering}:] see Section \ref{sec:pre-clustering}.
\item[\normalfont\texttt{- LMGP w/o Tracklet Split}:] no tracklet splitting using information from pre-clustering (Section \ref{sec:spatial-temporal-tracking-graph}, Splitting Tracklets).
\item[\normalfont\texttt{- LMGP w/o Enhanced Affinities}:] do not use pre-clustering in affinity cost computation (Eq. \ref{eq:appearance-affinity},
\ref{eq:pre-clustering-affinity}).
\item[\normalfont\texttt{- LMGP}:] our approach with everything enabled.
For the \textit{Campus} dataset we also provide as comparison \texttt{LMGP-DeepSort} using DeepSort~\cite{wojke2017simple} for generating tracklets.
Note that CenterTrack outperforms DeepSort on single camera benchmarks.
\end{packed_description}

\subsection{Results}
\vspace{-0.1in}
\begin{table}[!hbt]
\scalebox{0.63}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
Method& IDF1 $\uparrow$ & MOTA  $\uparrow$ & MT  $\uparrow$   & ML  $\downarrow$  & FP $\downarrow$ & FN $\downarrow$ & IDs $\downarrow$ \\ \Xhline{2\arrayrulewidth}
\small KSP-DO  \citep{chavdarova2018wildtrack}        & 73.2          & 69.6                               & 28.7          & 25.1        & 1095        & 7503        & 85           \\ 
\small KSP-DO-ptrack \citep{chavdarova2018wildtrack} & 78.4          & 72.2                               & 42.1         & 14.6         & 2007        & 5830        & 103          \\ 
\small GLMB-YOLOv3      \citep{9242263}       & 74.3          & 69.7                               & 79.5          & 21.6         & 424         & 1333        & 104          \\ 
\small GLMB-DO     \citep{9242263}      & 72.5          & 70.1                               & 93.6         & 22.8         & 960         & 990         & 107          \\ 
\small DMCT  \citep{you2020real}                   & 77.8          & 72.8                               & 61.0            & 4.9         & 91          & 126         & 42           \\ 
\small DMCT Stack  \citep{you2020real}              & 81.9          & 74.6                               & 65.9          & 4.9          & 114         & 107         & 21           \\ %\hline
\hdashline
\small LMGP w/o Pre-Clustering             & 79.4     & 73.6                        & 76.4      & 24.3     & 570   & 506  & 76    \\ 
\small LMGP w/o Tracklet Split & 92.4    & 89.7                        & 92.6      & 8.3     & 285  & 119  & 45   \\
\small LMGP w/o Enhanced Affinities & 95.1   & 94.8                         & 95.5       & 5.7      & 95  & 103  & 27   \\
\small LMGP            & \textbf{98.2} & \textbf{97.1}                      & \textbf{97.6} & \textbf{1.3} & \textbf{71} & \textbf{7}  & \textbf{12}  \\ \Xhline{2\arrayrulewidth}
\end{tabular}}
\vspace{-0.1in}
\caption{Our LMGP performance compared to state-of-the-art baselines on \textit{WILDTRACK}.}
\label{tab:multi-wildtrack}
\end{table}
\vspace{-0.2in}
%----------------
\begin{table}[!hbt]
  \centering
  \scalebox{0.62}{
  \begin{tabular}{c|c|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
   \multicolumn{1}{c|}{Sequence}   & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{MOTA $\uparrow$} & \multicolumn{1}{c|}{MOTP $\uparrow$} & \multicolumn{1}{c|}{MT $\uparrow$} & \multicolumn{1}{c|}{ML $\downarrow$} &
     \multicolumn{1}{c}{IDs $\downarrow$}\\ \Xhline{2\arrayrulewidth}
     \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L1}}}
     & HJMV  \citep{hofmann2013hypergraphs}                   &   91.7                        &     79.4                      &  94.7                         &  \textbf{0.0 }                      & 45 \\
     & STVH   \citep{wen2017multi}              &   95.1                        &          79.8                  &  \textbf{100.0}                         &  \textbf{0.0 }                      & 13  \\
     & MLMRF      \citep{lan2020semi}               &  96.8                         &       79.9                    &  \textbf{100.0}                        &   \textbf{0.0 }                    & \textbf{2} \\ 
     %\hline
     \hdashline
     & LMGP w/o Pre-Clustering                     &                  97.5       &        79.6                     &  96.3                         &   \textbf{0.0}                       & 6 \\
     & LMGP w/o Tracklet Split                      &    97.3                       &         82.1                  &                       97.2    &    \textbf{0.0}                      & 6 \\
     & LMGP w/o Enhanced Affinities                     &  97.6                         &    82.1                       &     98.1                     &        \textbf{0.0}                & 4 \\
     & LMGP                      &   \textbf{ 97.8}                     &          \textbf{82.4}                  &      \textbf{100.0}                     &   \textbf{0.0 }                      & \textbf{2} \\\Xhline{2\arrayrulewidth}

          \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L2}}}
     & HJMV  \citep{hofmann2013hypergraphs}                &   58.9                       &    66.0                         &  30.2                         &  2.3                      & 388  \\
     & STVH   \citep{wen2017multi}                       &     65.2                       &     61.8                    &  44.2                         & \textbf{ 0.0 }                       & 249  \\
     & MLMRF      \citep{lan2020semi}                  &      \textbf{ 72.1 }                  &     58.3                   &    \textbf{72.1 }                     &     2.3                     & 142 \\ %\hline
     \hdashline
     & LMGP w/o Pre-Clustering                      &                  66.8        &            64.3                &   67.4                        &    2.1                      &  158 \\
     & LMGP w/o Tracklet Split &    70.1                       &    68.5                       &             67.2              &    2.1                      & 97 \\
     & LMGP w/o Enhanced Affinities                      &  71.6                       &  \textbf{73.2 }                        &   68.2                       &   2.0                       & 81 \\
     & LMGP                               &  70.4   &    \textbf{73.2}                          &       69.6                    &      1.7                  & \textbf{75}\\\Xhline{2\arrayrulewidth}
          \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L3}}}
& HJMV  \citep{hofmann2013hypergraphs}              &   40.2                        &   49.5               &  29.6                         &  25.0                     & 123 \\
     &STVH   \citep{wen2017multi}                & 49.8                        &        63.0                   &    29.6                       &      20.5                    &   92\\
     & MLMRF      \citep{lan2020semi}                & \textbf{54.4}                         &    54.9                         &   36.4                        &      6.8                    & 82 \\
     %\hline
     \hdashline
     & LMGP w/o Pre-Clustering                     &     49.1                     &      55.7                      & 33.2                          &    13.6                      &  92 \\
     & LMGP w/o Tracklet Split                       & 52.7                          &   63.6                         &      33.4                     &   11.2                       & 86 \\
      & LMGP w/o Enhanced Affinities                      &         53.5                 &     64.7                     &    31.8                      &          8.7                & 82 \\
     & LMGP                      &              \textbf{54.4 }             &           \textbf{66.5}               &   \textbf{40.2}                        &  \textbf{5.3 }                       & \textbf{78}\\ 
\Xhline{2\arrayrulewidth}
\end{tabular}}
\vspace{-0.1in}
\caption{Our LMGP performance compared to other baselines in \textit{PETS-09}.}
\label{tab:pets09}
\end{table} 
%----------------
\vspace{-0.2in}
\begin{table}[!hbt]
  \centering
  \scalebox{0.65}{
  \begin{tabular}{c|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
   \multicolumn{1}{c|}{Sequence}   & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{MOTA $\uparrow$} & \multicolumn{1}{c|}{MOTP $\uparrow$} & \multicolumn{1}{c|}{MT $\uparrow$} & \multicolumn{1}{c}{ML $\downarrow$} \\ \Xhline{2\arrayrulewidth}
     \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{Garden 1}}}
     & HCT  \citep{xu2016multi}                   &   49.0                       &     71.9                     &  31.3                         &  6.3                     \\
     & STP   \citep{xu2017cross}              &   57                       &          75                  &  -                       & -                \\
     & TRACTA      \citep{he2020multi}               &  58.5                        &       74.3                    &  30.6                        &   1.6              \\ 
      & DyGLIP      \citep{quach2021dyglip}               &  71.2                      &       91.6                   &  31.3                        &   \textbf{0.0 }                   \\ 
     \hdashline
      & LMGP-DeepSort                    &   75.6                     &          93.4                 &      46.7                     &   1.6                      \\
     & LMGP                      &   \textbf{ 76.9}                     &          \textbf{95.9}                  &      \textbf{62.9}                     &   1.6                      \\\Xhline{2\arrayrulewidth}
          \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{Parking Lot}}}
     & HCT  \citep{xu2016multi}                &   24.1                      &    66.2                         &  6.7                         &  26.6                     \\
     & STP   \citep{xu2017cross}                       &     28                       &     68                    & -                      & -                \\
     & TRACTA      \citep{he2020multi}                  &     39.4              &     74.9                   &   15.5                   &     10.3                 \\ %\hline
       & DyGLIP      \citep{quach2021dyglip}               &  72.8                         &       \textbf{98.6}                  &  26.7                        &   \textbf{0.0 }                   \\ 
     \hdashline
      & LMGP-DeepSort                             &  76.7   &    98.0                       &       51.7                    &    5.1         \\
     & LMGP                               &  \textbf{78.1}   &    97.3                       &       \textbf{62.1}                    &     \textbf{0.0  }          \\\Xhline{2\arrayrulewidth}
  \end{tabular}}
\vspace{-0.1in}
\caption{Our LMGP performance compared to other baselines on \textit{Campus}.}
\label{tab:campus}
\end{table} 
\vspace{-0.2in}
We report quantitative results for \textit{WILDTRACK} in Table~\ref{tab:multi-wildtrack}, for \textit{PETS-09} in Table~\ref{tab:pets09}  and  for \textit{Campus} in Table~\ref{tab:campus}.
Some qualitative results are presented in Figures~\ref{fig:qualitative-results},\,\ref{fig:qualitative-results-campus} Appendix.

On \textit{WILDTRACK} we obtain almost perfect metric scores with \texttt{LMGP}. Our results on \textit{Campus} significantly outperform the state-of-the-art on both sequences even when using weak tracklets (DeepSort).
On \textit{PETS-09} we achieve comparable results.
We argue that the differing performance of our algorithms is mostly due to poor bounding boxes and camera calibration for \textit{PETS-09} and, to a lesser extent, for \textit{Campus}.
\subsection{Efficacy of Individual Components \& Ablations}
\label{sub:ablation-study}
To assess the performance of individual parts in our approach and their contribution to our overall performance, we give more experimental details.

\myparagraph{Ablations w.r.t.\ Pre-Clustering/Enhanced Affinities/Tracklet Splitting}
In Tables~\ref{tab:multi-wildtrack} and~\ref{tab:pets09} we report results of the ablated versions \texttt{LMGP w/o Pre-Clustering}, \texttt{LMGP w/o Tracklet Split} and \texttt{LMGP w/o Enhanced Affinities} of our solver. 
In most cases (except for \textit{S2-L1} of \textit{PETS-09}, where nearly perfect results can be obtained with any baseline), we see significant improvements w.r.t.\ all ablated versions of our solvers, validating the efficacy of all steps. 
\textit{The greatest performance drop can be observed by turning of the pre-clustering}, showing its important role for obtaining improved results.
More fine-grained ablations for the enhanced affinity costs can be found in Table~\ref{tab:temporal-costs-performance} and~\ref{tab:spatial-costs-performance} Appendix.

\myparagraph{Pre-Clustering Accuracy}
In Figure~\ref{fig:result-2Dclustering}, we report performance of our Pre-Clustering (Section~\ref{sec:pre-clustering}) for all considered datasets.
Since our Pre-Clustering is purely based on geometry, we also see experimentally that its performance is dependent upon the accuracy of bounding box coordinates.
In the high-quality \textit{WILDTRACK} dataset, we obtain almost perfect results.
For \textit{Campus} and \textit{PETS-09} we achieve precision higher than $80\%$.
We argue that the \textit{confident connection} in our pre-clustering helps in these more challenging and noisy settings.
More details on the reduction of ID-switch errors can be found in Table~\ref{tab:center-tracktor} Appendix.
\vspace{-0.15in}
\begin{figure}[!hbt]
\centering
\includegraphics[width=0.38\textwidth]{./imgs/Pre-Clustering_Performance_v2}
\vspace{-0.15in}
\caption{Our pre-clustering performance measured by accuracy, precision and recall w.r.t.\ correctly estimated correspondences between detections across cameras. On the top we give the total detections of objects in each dataset.
}
\label{fig:result-2Dclustering}
\vspace{-0.2in}
\end{figure}

\myparagraph{Joint Optimization Model}
In order to assess the performance of our joint spatio-temporal optimization model (Eq.\ref{eq:proposed-lmp}) as compared to a stage-wise optimization, we provide an experiment in  Table~\ref{tab:joint-spatial-temporal-optimize}.
The variant \texttt{LMGP w/o spatial edges} first solves an ordinary single view MOT problem. After obtaining computed single-camera trajectories, they are linked across cameras in a second step. To validate the effect of lifted long-range edges vs. a simpler model without them, we also provide an ablation \texttt{LMGP w/o lifted edges}. These ablations are tested on \textit{WILDTRACK} and \textit{S2-L1} of \textit{PETS-09}. The results 
indicate that significant improvement can be gained by optimizing jointly over temporal and camera affinities, especially in dense scenes like WILDTRACK. Also, the long-range edges contribute to better performance in both cases.
\begin{table}[!hbt]
\vspace{-0.1in}
  \centering
  \scalebox{0.6}{
  \begin{tabular}{c|c|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
    \multicolumn{1}{c|}{\small Dataset} & \multicolumn{1}{c|}{\small Method } & \multicolumn{1}{c|}{\small MOTA $\uparrow$} & \multicolumn{1}{c|}{\small IDF1 $\uparrow$} & \multicolumn{1}{c|}{\small MT $\uparrow$} &
    \multicolumn{1}{c|}{\small ML $\downarrow$} &
    \multicolumn{1}{c}{\small IDs $\downarrow$}\\ \Xhline{2\arrayrulewidth}
     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{0}{\small{\textit{WILDTRACK}} 
     }}}
     & \small {LMGP full}                      &   \textbf{97.1}                        &  \textbf{98.2}                         &  \textbf{97.6}                         &  \textbf{1.3}                   &  \textbf{12} \\
       & \small{LMGP w/o lifted edges}                      &   95.4                        &  96.4                         &  93.6                         &  2.7                  & 41  \\
     & \small{LMGP w/o spatial edges}                      &   93.2                        &  94.1                         &  91.7                         &  6.9                  & 85  \\
 \hline
          \multirow{2}{*}{\STAB{\rotatebox[origin=c]{0}{\small{\textit{S2-L1}}}}}
     & \small{LMGP full}                      &     \textbf{97.8}                      &  \textbf{82.4}                         &  \textbf{100.0}                        &  \textbf{0.0}                   &   \textbf{2}  \\
       & \small{LMGP w/o lifted edges}                      &  96.2                        &  81.1                         &  98.7                         &  1.3                    & 5 \\
     & \small{LMGP w/o spatial edges}                      &  95.6                        &  80.2                         &  98.7                         &  1.3                    & 8 \\
\Xhline{2\arrayrulewidth}
  \end{tabular}}
  \vspace{-0.1in}
  \caption{An ablation study of different edge types}
  \label{tab:joint-spatial-temporal-optimize}
\end{table} 
\vspace{-0.25in}
%   in two-steps compared to jointly reasoning through spatial-temporal edges.
\subsection{Discussion}
We have demonstrated that nearly perfect multiple object tracking results can be obtained in crowded scenes given the right conditions (as for \textit{WILDTRACK}), i.e.\ high bounding box quality and a large enough number of well-calibrated cameras observing the same scene.
Even when these conditions are not met, as in \textit{Campus} and \textit{PETS-09} which use old detectors, our \texttt{LMGP} still delivers better results than competitors in most cases.
% state-of-the-art results or better. 
Specifically, the \textit{pre-clustering is crucial in our framework} because it allows exploiting multi-camera information through repairing efficiently trajectories computed by single-camera trackers and can be used to enhance affinity costs.
Also, our lifted multicut model jointly optimizing over inter- and intra-camera affinities, short- and long-range interactions is essential and can effectively correct erroneous associations and continue trajectories which would be lost when only a single camera is used and severe occlusions are present.
% Given the improved tracklets from the pre-clustering phase, our global lifted multicut  model can effectively reason on inter- and intra-camera relations, correcting erroneous joins and continuing trajectories that would be lost when only observing with a single camera.
%\textcolor{red}{This correlation can be observed by considering the pre-clustering performance (Figure \ref{fig:result-2Dclustering}) and the results of \texttt{LMGP} on three datasets, i.e., better pre-clustering step implies better the total tracking performance in general.}
%Also our global optimization model jointly optimizing over inter- and intra-camera affinities is essential and can effectively correct erroneous joins and continue trajectories which would be lost when only observing with a single camera.



% \subsection{Dataset and Evaluation Metrics
% }
% % We use two different datasets for benchmark: WILDTRACK \cite{chavdarova2018wildtrack} and Campus \cite{xu2016multi}. The WILDTRACK until now is the large-scale dataset for the multi-camera setting with a dense group of $313$ pedestrians standing and walking. There are a total of $400$ frames at seven cameras were annotated together with its 3D positions where the first of $360$ frames used for training and the rest one for testing. The Campus is not as dense as WILDTRACK, with approximately $15 - 25$ pedestrians captured by four cameras in $3 - 4$ minutes, in which the first of $10\%$ video for training and the remainder for testing.  However, it is even more challenging than WILDTRACK due to staged property; thereby, several objects leave the surveillance area and come back after a long time but still get assigned with a unique ID number. We select three sequences in Campus for experiments: Garden-1, Garden-2 and Parking Lot. For both two datasets we use the provided detections for a fair comparison and validate performance on standard metrics in MOTChallenge \cite{leal2015motchallenge,milan2016mot16}. All baseline performances are extracted from original papers. 


% We use three different benchmark datasets: WILDTRACK~\cite{chavdarova2018wildtrack}, PETS-09~\cite{ellis2009pets2009} and Campus \cite{xu2016multi}. WILDTRACK currently is the largest-scale dataset for the multi-camera setting with a dense group of $313$ pedestrians standing and walking.
% There are a total of $400$ frames observed from seven cameras  that are annotated with 3D positions.
% The first $360$ of those frames are used for training and the rest for testing. In the PETS-09 dataset there are several scenarios with three levels of difficulty: low density (S2.L1) - $19$ objects in $795$ frames, medium density (S2.L2) - $43$ pedestrians spreading in $436$ frames and high density (S2.L3) - $44$ pedestrians moving together in $240$ frames.
% While PETS-09 is not as dense as WILDTRACK, its main challenge lies in poor video acquisition conditions with cameras far away from targets and low-quality bounding boxes. For both datasets, we use the provided detections for a fair comparison and validate performance on standard metrics in MOTChallenge~\cite{leal2015motchallenge,milan2016mot16}.
% All baseline performances are taken from the respective original papers. 

% % The Campus is not as dense as WILDTRACK, with approximately $15 - 25$ pedestrians captured by four cameras in $3 - 4$ minutes, in which the first of $10\%$ video for training and the remainder for testing.  However, it is even more challenging than WILDTRACK due to staged property; thereby, several objects leave the surveillance area and come back after a long time but still get assigned with a unique ID number. We select three sequences in Campus for experiments: Garden-1, Garden-2 and Parking Lot. For both two datasets we use the provided detections for a fair comparison and validate performance on standard metrics in MOTChallenge \cite{leal2015motchallenge,milan2016mot16}. All baseline performances are extracted from original papers. 
% % \croberto{This part needs to be updated since PETS09 is used..}

% % \myparagraph{Tracklet as a Node}
% % To generate the spatial-temporal lifted tracking graph $G$, we use CenterTrack~\cite{zhou2020tracking}, a recent state-of-the-art single-camera tracker, trained on the CrowdHuman dataset~\cite{shao2018crowdhuman}.
% % We create tracklets  for each camera.
% % These tracklets will be aligned again with the provided public detections to eliminate duplicate detections and to retain detections that were not tracked, e.g.\, due to occlusion.
% % Detailed parameters to train CenterTrack are provided in the Appendix. 

% % \myparagraph{Appearance Feature}
% % We integrate DG-Net \cite{zheng2019joint}, one of the best performing methods for re-identification to extract embedding vectors for detections.
% % To train DG-Net we process the training data and select a pre-clustering of unoccluded detections $C'_{b}$ for each object as described in equation \ref{eq:occlusion-filtering}.
% % We use the best models trained on Market-151~\cite{zheng2015scalable} and DukeMTMC-Reid~\cite{ristani2016performance} as the ``teacher network'' in DG-Net.

% % \myparagraph{Network Architecture}
% % Our formulation requires three networks: $f_{\mathrm{split}}$, $f_{\mathrm{spatial}}$, and $f_{\mathrm{temporal}}$ in order to split up initial tracklets, generating affinity costs for spatial and temporal edges correspondingly.
% % To this end we used three basic multi-layer deep networks.
% % The architecture is detailed in the appendix.
% % The training data for $f_{\mathrm{spatial}}$ and $f_{\mathrm{temporal}}$ is prepared through a sampling strategy as described in the appendix.
% % Training data for $f_{split}$ is obtained by running the trained CenterTrack on the validation set.
% % We use a modified F1 loss function~\cite{johnson2019survey} during the training process to mitigate problems caused by training with Adam~\cite{kingma2014adam} with imbalanced training data.
% % The learning rate is $0.001$.
% % We also use the radius $r = 2$ and $3$ meters in WILDTRACK and PETS09 correspondingly to compute 3D geometry costs and pre-clustering. 

% %  $f_{filter}$ is trained with $5$ epochs and two others are trained with $100$ epochs. They all

% % %------------------------------------------
% % \subsection{Baseline Experiments}
% % \textcolor{red}{Referring baseline methods used to compare in each dataset. }
% %------------------------------------------

% \subsection{Performance of Pre-clustering}
% \label{sec:pre_clustering_performance}
% We investigate robustness and accuracy of our pre-clustering. 
% We want to emphasize that this step is critical for performance since it allows us to correct ID-switch errors made during tracklet generation and for obtaining better affinity costs due to incorporating multiple detections from different cameras of the same object.
% Figure \ref{fig:result-2Dclustering} summarizes our main results across different sequences in WILDTRACK and PETS09 on various metrics measured on the total processed objects.
% We also show the total number of objects handled by our algorithm for each sequence, computed by counting the total independent pedestrians over the whole data frames.
% Each object is considered correct if our pre-clustering could retrieve all of its instances across different views.
% The empirical results indicate high performance of our algorithm on WILDTRACK with up to $99\%$ on different metrics.
% On PETS09 we obtain significantly lower accuracy and recall when increasing target density.
% However, the precision value is still stable (above $80\%$).
% The reason behind this observation lies in the poor bounding box and camera poses, which influences whether our 3D geometry processing is accurate.
% Fortunately, even under heavy perturbations our scheme's pre-clustering can alleviate errors, resulting in a robust performance in terms of precision.

% \begin{figure}[!hbt]
% \centering
% \includegraphics[width=0.5\textwidth]{Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/imgs/Pre-Clustering_Performance_v2}
% \caption{The performance of our pre-clustering over datasets. 
% For each method we give accuracy, precision and recall w.r.t.\ correctly estimated correspondences between detections across cameras. 
% On the top we give the total number of observed people.
% }
% \label{fig:result-2Dclustering}
% \end{figure}
%------------------------------------------


% \subsection{Multi-Camera Benchmark}
% % We conduct several experiments on the multi-people multi-camera tracking datasets  WILDTRACK and PETS-09 to assess our proposed tracking pipeline.
% We report our tracking results in Table~\ref{tab:multi-wildtrack} and Table~\ref{tab:campus}, together with the best-performing methods.
% % All measurements follow the evaluation protocol of the respective benchmark, \ie we use the publicly provided detections, and measure the accuracy on the 3D ground space for WILDTRACK, resp.\ average over 2D single camera results on PETS09.
% To assess the importance of the different components of our work, we perform ablation studies, where we analyze the impact of our pre-clustering procedure  (LMGP w/o Pre-Clustering, Section~\ref{sec:cluster_effect}), the tracklet splitting (LMP w/o Graph Process, Section~\ref{sec:graph_filter}), and disabling pre-clustering in affinity cost computing (LMP w/o Enhance Affinities, Section \ref{sec:enhanced-affinity}).
% Next, we compare our full method (LMGP) to the state of the art in Section~\ref{sec:compare_with_baselines}. Finally, we demonstrate the benefit of our global lifted multicut formulation in Section \ref{sec:variation-optimize}.

% %The table \ref{tab:multi-wildtrack} and \ref{tab:campus} present the most important experiments that compare our performance to the latest multi-people multi-camera baselines on WILDTRACK and Campus dataset. We measured all metrics following the same settings for each dataset, e.g., 3D ground space estimating on WILDTRACK and averaging over single cameras on Campus.
% % Finally, we evaluate our performance on the multi-people multi-camera tracking datasets  WILDTRACK and PETS09. To this end, we follow the evaluation protocol of the respective benchmark, \ie we use detections provided by the benchmarks, and measure the accuracy on the 3D ground space for WILDTRACK, resp.\ average over 2D single camera results on PETS09. Table \ref{tab:multi-wildtrack} and Table \ref{tab:campus} show the results achieved by our method and report the best performing competing methods on the respective benchmarks. Overall, we see that our baseline without using 3D information (LMGP w/o 3D), \ie without our pre-clustering (Section \ref{sec:pre-clustering}) performs on pair with competing methods on WILDTRACK, but is behind state of the art on PETS09 on the more crowded sequences (S2-L2 and S2-L3). Using pre-clustering, but without correcting tracking errors (Section  \ref{sec:spatial-temporal-tracking-graph}, Splitting Tracklets) improves IDF1 on WILDTRACK considerably by more than 10 percentage points, already outperforming state of the art. Likewise the pre-clustering reduced the number of ID switches by about 45\%. It also enables to heavily reduce false positives (more than 50\%) and false negatives (about 75\%), resulting in a MOTA improvement by $16$ percentage points. The PETS09 dataset shows that the gain by the pre-clustering increases with the object density. The improvement in terms of MOTA is between $0.2$ points for a low crowded scene (S2-L1), up to more than $9$ points on a very crowded scene (S2-L3) with frequent occlusions, which shows that the pre-clustering is crucial to obtain stable results, especially in crowded scenes.
% % Finally, splitting of tracklets at likely identity switches further increases all measured tracking metrics across all datasets. 
% % On WILDTRACK, all tracking metrics outperform state of the art by a large margin, \eg compared to \cite{you2020real}, $98.2$ IDF1 vs $81.9$ IDF1, $7$ FN vs $107$ FN, or $97.3$ MOTA vs $74.6$ MOTA. On PETS-09, our methods performs state of the art.

% % \begin{table}[!hbt]
% % \scalebox{0.6}{
% % \begin{tabular}{c|c|c|c|c|c|c|c}
% % \Xhline{2\arrayrulewidth}
% % Method& IDF1 $\uparrow$ & MOTA  $\uparrow$ & MT  $\uparrow$   & ML  $\downarrow$  & FP $\downarrow$ & FN $\downarrow$ & IDs $\downarrow$ \\ \Xhline{2\arrayrulewidth}
% % Deep Occlusion + KSP  \cite{chavdarova2018wildtrack}        & 73.2          & 69.6                               & 28.7          & 25.1        & 1095        & 7503        & 85           \\ 
% % Deep Occlusion + KSP + ptrack \cite{chavdarova2018wildtrack} & 78.4          & 72.2                               & 42.1         & 14.6         & 2007        & 5830        & 103          \\ 
% % YOLOv3+MV-GLMB-OC      \cite{9242263}       & 74.3          & 69.7                               & 79.5          & 21.6         & 424         & 1333        & 104          \\ 
% % Deep Occlusion  + GLMB     \cite{9242263}      & 72.5          & 70.1                               & 93.6         & 22.8         & 960         & 990         & 107          \\ 
% % DMCT  \cite{you2020real}                   & 77.8          & 72.8                               & 61.0            & 4.9         & 91          & 126         & 42           \\ 
% % DMCT Stack  \cite{you2020real}              & 81.9          & 74.6                               & 65.9          & 4.9          & 114         & 107         & 21           \\
% % LMGP (w/o Pre-clustering)             & 79.4     & 73.6                        & 76.4      & 24.3     & 570   & 506  & 76    \\ 
% % LMGP (w/o Graph Process) & 92.4    & 89.7                        & 92.6      & 8.3     & 285  & 119  & 45   \\
% % LMGP (w/o Enhance Affinities) & 95.1    & 94.8                        & 95.5      & 5.7     & 95  & 103  & 27   \\
% % LMGP (Full)             & \textbf{98.2} & \textbf{97.3}                      & \textbf{97.6} & \textbf{1.3} & \textbf{44} & \textbf{7}  & \textbf{11}  \\ \Xhline{2\arrayrulewidth}
% % \end{tabular}}
% % \vspace{0.05in}
% % \caption{Our tracking performance compared to other moderns multi-camera methods in WILDTRACK.}
% % \label{tab:multi-wildtrack}
% % \end{table}

% \begin{table}[!hbt]
% \scalebox{0.63}{
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \Xhline{2\arrayrulewidth}
% Method& IDF1 $\uparrow$ & MOTA  $\uparrow$ & MT  $\uparrow$   & ML  $\downarrow$  & FP $\downarrow$ & FN $\downarrow$ & IDs $\downarrow$ \\ \Xhline{2\arrayrulewidth}
% \small KSP-DO  \citep{chavdarova2018wildtrack}        & 73.2          & 69.6                               & 28.7          & 25.1        & 1095        & 7503        & 85           \\ 
% \small KSP-DO-ptrack \citep{chavdarova2018wildtrack} & 78.4          & 72.2                               & 42.1         & 14.6         & 2007        & 5830        & 103          \\ 
% \small GLMB-YOLOv3      \citep{9242263}       & 74.3          & 69.7                               & 79.5          & 21.6         & 424         & 1333        & 104          \\ 
% \small GLMB-DO     \citep{9242263}      & 72.5          & 70.1                               & 93.6         & 22.8         & 960         & 990         & 107          \\ 
% \small DMCT  \citep{you2020real}                   & 77.8          & 72.8                               & 61.0            & 4.9         & 91          & 126         & 42           \\ 
% \small DMCT Stack  \citep{you2020real}              & 81.9          & 74.6                               & 65.9          & 4.9          & 114         & 107         & 21           \\ %\hline
% \hdashline
% \small LMGP w/o Clusters             & 79.4     & 73.6                        & 76.4      & 24.3     & 570   & 506  & 76    \\ 
% \small LMGP w/o Graph Process & 92.4    & 89.7                        & 92.6      & 8.3     & 285  & 119  & 45   \\
% \small LMGP w/o Enhanced Affinities & 95.1   & 94.8                         & 95.5       & 5.7      & 95  & 103  & 27   \\
% \small LMGP            & \textbf{98.2} & \textbf{97.1}                      & \textbf{97.6} & \textbf{1.3} & \textbf{71} & \textbf{7}  & \textbf{12}  \\ \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \vspace{0.05in}
% \caption{Our LMGP performance compared to state-of-the-art baselines on \textit{WILDTRACK}.}
% \label{tab:multi-wildtrack}
% \end{table}
% \vspace{-0.2in}
% %%%%%%%%%%%%%%%%%%
% \begin{table}[!hbt]
%   \centering
%   \scalebox{0.62}{
%   \begin{tabular}{c|c|c|c|c|c|c}
% \Xhline{2\arrayrulewidth}
%   \multicolumn{1}{c|}{Sequence}   & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{MOTA $\uparrow$} & \multicolumn{1}{c|}{MOTP $\uparrow$} & \multicolumn{1}{c|}{MT $\uparrow$} & \multicolumn{1}{c|}{ML $\downarrow$} &
%      \multicolumn{1}{c}{IDs $\downarrow$}\\ \Xhline{2\arrayrulewidth}
%      \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L1}}}
%      & HJMV  \citep{hofmann2013hypergraphs}                   &   91.7                        &     79.4                      &  94.7                         &  \textbf{0.0 }                      & 45 \\
%      & STVH   \citep{wen2017multi}              &   95.1                        &          79.8                  &  \textbf{100.0}                         &  \textbf{0.0 }                      & 13  \\
%      & MLMRF      \citep{lan2020semi}               &  96.8                         &       79.9                    &  \textbf{100.0}                        &   \textbf{0.0 }                    & \textbf{2} \\ 
%      %\hline
%      \hdashline
%      & LMGP w/o Clusters                     &                  97.5       &        79.6                     &  96.3                         &   \textbf{0.0}                       & 6 \\
%      & LMGP w/o Graph Process                      &    97.3                       &         82.1                  &                       97.2    &    \textbf{0.0}                      & 6 \\
%      & LMGP w/o Enhanced Affinities                     &  97.6                         &    82.1                       &     98.1                     &        \textbf{0.0}                & 4 \\
%      & LMGP                      &   \textbf{ 97.8}                     &          \textbf{82.4}                  &      \textbf{100.0}                     &   \textbf{0.0 }                      & \textbf{2} \\\Xhline{2\arrayrulewidth}

%           \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L2}}}
%      & HJMV  \citep{hofmann2013hypergraphs}                &   58.9                       &    66.0                         &  30.2                         &  2.3                      & 388  \\
%      & STVH   \citep{wen2017multi}                       &     65.2                       &     61.8                    &  44.2                         & \textbf{ 0.0 }                       & 249  \\
%      & MLMRF      \citep{lan2020semi}                  &      \textbf{ 72.1 }                  &     58.3                   &    \textbf{72.1 }                     &     2.3                     & 142 \\ %\hline
%      \hdashline
%      & LMGP w/o Clusters                      &                  66.8        &            64.3                &   67.4                        &    2.1                      &  158 \\
%      & LMGP w/o Graph Process                     &    70.1                       &    68.5                       &             67.2              &    2.1                      & 97 \\
%      & LMGP w/o Enhanced Affinities                      &  71.6                       &  \textbf{73.2 }                        &   68.2                       &   2.0                       & 81 \\
%      & LMGP                               &  70.4   &    \textbf{73.2}                          &       69.6                    &      1.7                  & \textbf{75}\\\Xhline{2\arrayrulewidth}
%           \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{S2-L3}}}
% & HJMV  \citep{hofmann2013hypergraphs}              &   40.2                        &   49.5               &  29.6                         &  25.0                     & 123 \\
%      &STVH   \citep{wen2017multi}                & 49.8                        &        63.0                   &    29.6                       &      20.5                    &   92\\
%      & MLMRF      \citep{lan2020semi}                & \textbf{54.4}                         &    54.9                         &   36.4                        &      6.8                    & 82 \\
%      %\hline
%      \hdashline
%      & LMGP (w/o Clusters)                     &     49.1                     &      55.7                      & 33.2                          &    13.6                      &  92 \\
%      & LMGP (w/o Graph Process)                       & 52.7                          &   63.6                         &      33.4                     &   11.2                       & 86 \\
%       & LMGP (w/o Enhanced Affinities)                      &         53.5                 &     64.7                     &    31.8                      &          8.7                & 82 \\
%      & LMGP (Full)                      &              \textbf{54.4 }             &           \textbf{66.5}               &   \textbf{40.2}                        &  \textbf{5.3 }                       & \textbf{78}\\ 
% \Xhline{2\arrayrulewidth}
%   \end{tabular}}
% \vspace{0.05in}
%   \caption{Our LMGP performance compared to other baselines in \textit{PETS-09}.}
%     \label{tab:pets09}
% \end{table} 

% %%%%%%%%%%%%%%%%%%
% \begin{table}[!hbt]
%   \centering
%   \scalebox{0.8}{
%   \begin{tabular}{c|c|c|c|c|c}
% \Xhline{2\arrayrulewidth}
%   \multicolumn{1}{c|}{Sequence}   & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{MOTA $\uparrow$} & \multicolumn{1}{c|}{MOTP $\uparrow$} & \multicolumn{1}{c|}{MT $\uparrow$} & \multicolumn{1}{c|}{ML $\downarrow$} \\ \Xhline{2\arrayrulewidth}
%      \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{Garden 1}}}
%      & HCT  \citep{xu2016multi}                   &   49.0                       &     71.9                     &  31.3                         &  6.3                     \\
%      & STP   \citep{xu2017cross}              &   57                       &          75                  &  -                       & -                \\
%      & TRACTA      \citep{he2020multi}               &  58.5                        &       74.3                    &  30.6                        &   1.6              \\ 
%       & DyGLIP      \citep{quach2021dyglip}               &  71.2                      &       91.6                   &  31.3                        &   \textbf{0.0 }                   \\ 
%      \hdashline
%      & LMGP                      &   \textbf{ 76.9}                     &          \textbf{95.9}                  &      \textbf{62.9}                     &   1.6                      \\\Xhline{2\arrayrulewidth}
%           \multirow{5}{*}{\STAB{\rotatebox[origin=c]{0}{Parking Lot}}}
%      & HCT  \citep{xu2016multi}                &   24.1                      &    66.2                         &  6.7                         &  26.6                     \\
%      & STP   \citep{xu2017cross}                       &     28                       &     68                    & -                      & -                \\
%      & TRACTA      \citep{he2020multi}                  &     39.4              &     74.9                   &   15.5                   &     10.3                 \\ %\hline
%       & DyGLIP      \citep{quach2021dyglip}               &  72.8                         &       \textbf{98.6}                  &  26.7                        &   \textbf{0.0 }                   \\ 
%      \hdashline
%      & LMGP                               &  \textbf{78.1}   &    97.3                       &       \textbf{62.1}                    &     \textbf{0.0  }          \\\Xhline{2\arrayrulewidth}
%   \end{tabular}}
% \vspace{0.05in}
%   \caption{Our LMGP performance compared to other baselines on \textit{Campus}.}
%     \label{tab:campus}
% \end{table} 


% \croberto{Report IDF1 aswell, change column order. IDF1, then MOTA, then MOTP,..}
% %---------------------------------------
% \subsubsection{Influence of Pre-Clustering}
% \label{sec:cluster_effect}
% % We investigate the influence of our 2D clustering, denoted as LMP (w/o Clusters). Specifically, 
% For this experiment, we skip the 3D geometry based pre-clustering in pre-processing of the tracking graph and computation of affinities; only our global lifted multicut formulation and tracklet-based graph is employed. 
% Table~\ref{tab:campus} shows that we achieve competitive performance on PETS09 for the sequence S2-L1. Also, Table~\ref{tab:multi-wildtrack} shows that we hold the second rank on WILDTRACK behind DMCT~\cite{you2020real} for IDF1/MOTA and IDs. We believe that due to CenterTrack computing good initial trajectories, our method could obtain good IDF1 and MOTA scores, while the low IDs come from our optimization formulation that incorporates long-range interactions.
% However, the values on IDs, FP and FN are much lower than DMCT's.
% This is to be expected, since DMCT exploits correspondences between detections in 3D across cameras, which we deactivated in this ablation setting. 


% %We first conduct an ablation study to investigate the influence of our 2D clustering effects, namely LMP (w/o 3D). In specific, we ignore using this module in pre-processing the graph tracking and composing affinity costs; only our novel formulation and tracklet-based graph are employed. It could be observed that we achieved a competitive benchmark on PETS09 for all sequences and hold the second rank in WILDTRACK after the DMCT approach, especially on IDF1/MOTA and IDs. We believe that the two first metrics (IDF1/MOTA) take advantage of CenterTrack to form a good initialization tracking while the low IDs coming from our optimization formulation with the long-range interaction are considered. However, our values on both IDs, FP and FN, are still much lower than DMCT; the method has used 2D correspondences at each frame to handle target trackings.
% \vspace{-0.1in}
% \subsubsection{Influence of Splitting Tracklets}
% \label{sec:graph_filter}
% We next validate how the tracklet splitting affects the final performance filtering. To this end, we activate again the pre-clustering during the spatial-temporal affinity computation, but keep all initial tracklets as generated by CenterTrack.
% % This tracker is denoted as LMP w/o Graph Process.
% As the evaluations show all metrics are improved, for example, IDF1 increases significantly from $79.4\%$ to $92.4\%$ on WILDTRACK.
% % Similarly, FP, FN, and IDs total errors decrease significantly from 570, 506, and 76 down to 285, 119, and  45, respectively.
% A similar trend also occurs on PETS09.
% % On S2-L2, MOTA and IDs improves from $66.8\%$ and $158$ to $70.1\%$ and $97$, respectively.
% These evidences confirm that our novel affinities derived from pre-clustering lead to more discriminative spatial and temporal metrics as inter-camera correspondences are exploited. 
% % The results on both datasets suggest that our 2D clustering leads to more discriminative spatial and temporal affinities by carefully exploiting inter-camera correspondences.
% %We provide further experiments for such changes in ablation study. 
% However, several metrics such as FP, FN, or IDs are still much lower than DMCT's.
% We believe that this problem can by explained by ID-switch errors in the tracklets, which are not eliminated, leading to error propagation phenomenon.

% % We also note that for the  sparsely crowded sequence (S2-L1) features are less ambiguous so that tracklets from tracktor can hardly be improved.  


% %These limitations are intuitively caused by the graph's attribute, thereby several ID-Switches errors generated by the tracklets were not eliminated properly, leading to error propagation during handling tracking results.


% % We next validate how the global graph filtering affects the final performance by only incorporating our clustering into computing spatial-temporal affinity step; an initial graph with tracklets from CenterTrack will be kept. This option is denoted as LMP w/o Graph Process. The results on both datasets suggest that using clustering results makes a massive increase for all metrics. For example, the IDF1 increases from $81.9\%$ up to $92.4\%$ on WILDTRACK. Similarly, FP, FN, and IDs' total errors decreases significantly from 570, 506, and 76 down to 285, 119, and  45. A similar trend also occurs on PETS09; for instance, the IDF1 improvement of $x\%$ and IDs decreases down to $y$. We argue that the underlying reason lies in enhancing the quality of space and time affinity costs through using further constraints from the 2D correspondences step. We provide further experiments for such changes in ablation study. Unfortunately, several existing metrics as FP, FN, or IDs are still much lower than DMCT. These limitations are intuitively caused by the graph's attribute, thereby several ID-Switches errors generated by the tracklets were not eliminated properly, leading to error propagation during handling tracking results.
% \vspace{-0.1in}
% \subsubsection{Influence of Enhanced Affinity Costs}
% \label{sec:enhanced-affinity}
% For this setting, we only use the pre-clustering component in pre-processing tracking graph and deactivate it in affinities composing (Equations \ref{eq:appearance-affinity},\ref{eq:pre-clustering-affinity}). It could be observed that this setting improves in most cases compared to not pre-process tracking graph, especially in ID-switch errors. 
% % In WILDTRACK and S2-L2, for example, the IDs drop from $45 \text{ and } $95 to $27 \text{ and } $81, respectively.  Similarly, FP and FN also benefit with a huge improvement, from $285 \text{ and }119$ down to $95 \text{ and }103$ on WILDTRACK. 
% We interpret this phenomenon as a result of the tracking graph's quality, which harnesses advantages of tracklets when ID-switch problems are adequately treated. However, obtained results compared with fully setting, i.e., using pre-clustering on both graph construction and affinity cost designing, are still much lower because the better costs from pre-clustering imply a better overall efficiency.

% \vspace{-0.1in}
% \subsubsection{Comparison with Baselines}
% \label{sec:compare_with_baselines}
% Finally, we analyze our complete configurations where all components are integrated:
% splitting tracklets, designing affinity costs using pre-clustering and optimizing our novel spatial-temporal lifted multicut formulation.
% It can be seen that we achieve state-of-the-art performance with a large margin compared to all baselines on WILDTRACK.
% For instance, we outperform DMCT~\cite{you2020real} by approximately $17$ percentage points on IDF1, and IDs is decreased by about $50\%$ with only 11 errors.
% %
% Likewise on PETS09, our full system achieves a consistent improvement on most metrics. However, our margin in WILDTRACK is much larger in PETS09. We argue that the significant improvement on WILDTRACK is due to more precise detections (PETS-09 uses DPM~\cite{felzenszwalb2008discriminatively}), resulting in a more accurate pre-clustering (Figure \ref{fig:2Dclustering}).
% Also the larger distances of people to the camera in PETS09 cause more 3D localization errors.
% % In short, we conclude that the state of the art performance of our proposed method reflects several factors in our framework, from the graph construction, discriminative affinities, and an expressive optimization formulation.
% In the Appendix, we further compare LMGP with single camera trackers, discuss computational time and show qualitative tracking results.

% %Similarly, on PETS09, we establish new milestones for all metrics, with $x\%$ for MOTP and $y$ for IDs. 




% % Finally, we analyze our complete configurations where all components are integrated as filtering the tracking graph, designing affinity costs using 2D clustering, and optimizing our novel space-time formulation. It can be seen that we obtain state-of-the-art performance with a large margin compared to all baselines. For instance, we outperform approximately $17\%$ on IDF1 and low IDs with only 11 errors than DMCT on WILDTRACK. Similarly, on PETS09, we establish new milestones for all metrics, with $x\%$ for MOTP and $y$ for IDs. We conclude that this superior performance reflects several factors in our framework, from graph construction step, quality affinity costs, and an expressive optimization formulation. In ablation study, we also show some our qualitative tracking results on two datasets. Besides, the time consuming factor is also discussed.

% %-----------------------------------------
% %------------------------------------------------------------------------

% % \subsection{Single-Camera Benchmark}
% % We provide experimental results on WILDTRACK compared to three modern single camera pedestrian tracking methods.
% % As we mentioned, even with the best methods, the single-camera approach is still insufficient under severe occlusions.
% % Considering large improvements on all metrics, we argue that the multi-camera strategy convincingly improves upon the single-camera one in crowded settings.

% % \begin{table}[!hbt]
% % \scalebox{0.6}{
% % \begin{tabular}{c|c|c|c|c|c|c|c}
% % \Xhline{2\arrayrulewidth}
% % Method& IDF1 $\uparrow$ & MOTA  $\uparrow$ & MT  $\uparrow$   & ML  $\downarrow$  & FP $\downarrow$ & FN $\downarrow$ & IDs $\downarrow$ \\ \Xhline{2\arrayrulewidth}
% % Deep MCD + KSP + ptrack \cite{chavdarova2018wildtrack} & 64.3          & 52.4                              & 83.4         & 10.7         & 1023        & 2239        & 711          \\ 
% % Tracktor++   \cite{bergmann2019tracking}         & 65.0          & 60.4                               & 68.3          & 8.7        & 819         & 637        & 272          \\
% % CenterTrack   \cite{zhou2020tracking}    & 67.4         & 67.5                               & 74.6         & 3.4        & 649        & 494         & 278          \\ 
% % LMGP (Full)             & \textbf{97.6} & \textbf{96.8}                      & \textbf{96.3} & \textbf{2.1} & \textbf{60} & \textbf{10}  & \textbf{44}  \\ \Xhline{2\arrayrulewidth}
% % \end{tabular}}
% % \vspace{0.05in}
% % \caption{Our tracking performance compared to state of the art single camera methods on WILDTRACK.}
% % \label{tab:single-camera}
% % \end{table}
% % % \section{Discussion}
% % % \textcolor{red}{Keypoint makes our method outperforms all current works with a large margin: (1) pre-clustering, (2) tracklets from modern 2D Tracker (CenterTrack), (3) Good formulation with Lifted-Cut and (4) state-of-the-art Re-identification features as well as proposed motion features.}
% % %------------------------------------------------------------------------
% % % \section{Conclusion}
% % % In this work, we contribute a novel space-time lifted multi-cut formulation using multi-camera to address tracking problems under severe occluded scenes. Along with it, a novel 2D correspondences clustering is proposed by exploiting 3D geometry constraints across multi-views. The experimental results have proven how our proposed method is effective with an outstanding performance compared to other baselines.

% \subsection{Influence of Joint Spatial-Temporal Reasoning}
% \label{sec:variation-optimize}
% Our lifted multicut formulation optimizes simultaneously intra-camera (temporal edges) and inter-camera (spatial edges) associations.
% We validate influences of this approach on WILDTRACK and the first sequence S2-L1 on PETS-09. Given the tracking graph $G$ processed with ID-Switch errors and our enhanced affinity costs, we first partition the graph $G$ by optimizing individually on each view first and then linking derived clusters across cameras in the next step (LMGP-Individual). As compared with our default configuration (LMGP-Joint) in Table \ref{tab:joint-spatial-temporal-optimize}, the LMGP-Individual achieves significantly lower performance, specifically on WILDTRACK. We explain this phenomenon  through occlusion levels in each data.
% In WILDTRACK, we have several severely occluded artifacts in some cameras,  inducing a higher error in the spatial linking step.
% These errors are retained in the next step, resulting in significant errors overall. In S2-L1, on the other hand, where the number of tracking targets is not large and the occlusion level is comparatively low, the data association based on spatial edges can still track most objects satosfactorily.
% % However, separate data reasoning is less successful than the joint optimization approach in terms of IDs. 
% % To summarize, we conclude that our formulation that optimizes the global spatial-temporal tracking graph is both consistent and efficient.

% \begin{table}[!hbt]
%   \centering
%   \scalebox{0.7}{
%   \begin{tabular}{c|c|c|c|c|c|c}
% \Xhline{2\arrayrulewidth}
%     \multicolumn{1}{c|}{\small Method} & \multicolumn{1}{c|}{\small Data } & \multicolumn{1}{c|}{\small MOTA $\uparrow$} & \multicolumn{1}{c|}{\small IDF1 $\uparrow$} & \multicolumn{1}{c|}{\small MT $\uparrow$} &
%     \multicolumn{1}{c|}{\small ML $\downarrow$} &
%     \multicolumn{1}{c}{\small IDs $\downarrow$}\\ \Xhline{2\arrayrulewidth}
%      \multirow{2}{*}{\STAB{\rotatebox[origin=c]{0}{\small{LMGP-Joint} 
%      }}}
%      & \small {WILDTRACK}                      &   97.1                        &  98.2                         &  97.6                         &  1.3                   &  12 \\
%      & \small{S2-L1}                      &     97.8                      &  82.4                         &  100.0                        &  0.0                   &   2  \\
%  \hline
%           \multirow{2}{*}{\STAB{\rotatebox[origin=c]{0}{\small{LMGP-Individual}}}}
%      & \small{WILDTRACK}                      &   93.2                        &  94.1                         &  91.7                         &  6.9                  & 85  \\
%      & \small{S2-L1}                      &  95.6                        &  80.2                         &  98.7                         &  1.3                    & 8 \\
% \Xhline{2\arrayrulewidth}
%   \end{tabular}}
%   \vspace{0.05in}
%   \caption{Our performance as optimizing in two-steps compared to jointly reasoning through spatial-temporal edges.}
%   \label{tab:joint-spatial-temporal-optimize}
% \end{table} 

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/introduction.tex <==
\section{Introduction}
\begin{figure}[!hbt]
\centering
\includegraphics[width=0.48\textwidth]{./imgs/Overview_Ideas_v5.png}
\caption{
Multi-camera tracking with four overlapping cameras. A target object (red rectangle) is occluded at Cam 3 but is still observed at Cam 1, Cam 2, and Cam 4. Taking this correspondence into account (red arrow), we can recover a missing bounding box at Cam 3 (red dashed arrow).}
\label{fig:teaser_crop}
\vspace{-0.2in}
\end{figure}
Multiple object tracking (MOT), i.e., \ extracting motions of objects moving through a scene, is a fundamental primitive for high-level understanding information in videos.
The most common approach to MOT is the tracking-by-assignment paradigm, in which first detection boxes are computed for the objects of interest in each timeframe, and second, a data association is performed by linking detections of the same objects to each other.
In the most popular setting, a single camera faces a scene and the data association links detections in different timeframes to each other ~\citep{bewley2016simple, wojke2017simple, chu2019famnet,bergmann2019tracking}.
However, even though a large body of research has been devoted to MOT with a single camera, large and crowded scenes still cannot be tracked faithfully, and errors occur mainly in the data association step.
These errors most often are caused by partial visibility (or even occlusion) and indistinguishability of objects.

One possibility of improving performance has been to use multiple cameras facing the same scene but from different angles (Figure \ref{fig:teaser_crop}).
In this setting, partial visibility and indistinguishability are less severe since an object may be occluded in a single camera but may still be fully observed by another camera. Leveraging this property, recent papers have pursued two principal approaches: \textit{single view-based} and \textit{centralized representation} methods. In the first strategy \cite{xu2017cross,he2020multi,lan2020semi,quach2021dyglip}, a two-step procedure is followed: 1) generating local tracklets of all the targets within each camera; 2) matching local tracklets that belong to the same target across cameras through computing affinity costs and using a global optimization framework. While this framework brings benefits via a reduced hypothesis space and allows to design motion-based features, its main drawbacks lie in ID-Switch errors contained inside local tracklets, i.e., detections of distinct objects are grouped into the same trajectory (Figure \ref{fig:split-tracklet}a). As a result, these errors will propagate throughout the tracking graph,
affecting the total performance. \textit{The centralized representation} approach \cite{zhang2019wide,you2020real} on the other hand, is not plagued by such obstacles since each node in the tracking graph is an occupancy map (not a tracklet), which is estimated from all detections at each timeframe. Unfortunately, the cost of the data association step is increased due to a huge state space of variables and integrating advances from single-camera methods is more complicated.


% While an object may be occluded in a single camera, another camera may still capture the object in full.
% While two objects may be too similar to tell them apart, multiple cameras can potentially triangulate their 3D-positions and this additional spatial feature may be discriminative.
% However, the computational complexity of the data association step is increased: Not only are detections linked across timeframes (temporal association), they must be linked across frames at the same timesteps but observed by different cameras (spatial association).
% On top of that, temporal and spatial associations must lead to tracks that are consistent with each other.

In this work, we propose a method that follows the \textit{single view-based approach} but integrates concepts from the centralized representation paradigm. Our motivation for this design choice is to harness the great progress made in single-camera tracking while at the same time effectively addressing limitations encountered in prior studies such as ID-Switch errors by exploiting \textit{centralized representation} ideas through our novel pre-clustering step.
% \roberto{We propose a method that follows a \textit{single view-based approach}, but integrates concepts from the centralized representation ideas.}. Our motivation for this choice is to harness the great progress made in single-camera tracking. However, we can effectively address limitations encountered in prior studies such as ID-Switch errors by exploiting \textit{centralized representation} ideas through our novel pre-clustering step.
Specifically, the corresponding images from the pre-clustering step (i.e.\ our occupancy map) allow us to break up initial tracklets generated by single-camera trackers at ID-Switch errors and establish precise affinity costs for both temporal and spatial affinities (Subsection \ref{sub:ablation-study}). On top of that, a novel spatial-temporal optimization model for the data association is employed, which takes into account both short- and long-range temporal interactions of objects detected by a single camera as well as spatial interactions between cameras in a single framework (Table \ref{tab:joint-spatial-temporal-optimize}). The experimental findings show that, given the right conditions, with a multiple-camera environment and precise boundary detections, our method leads to a nearly optimal solution for multiple object tracking using multiple cameras (Table \ref{tab:multi-wildtrack}).

% In this work we propose an elegant novel spatial-temporal optimization model for the data association step for multi-camera MOT.
% Our model is based on the lifted multicut problem~\cite{keuper2015lifted}.
% It takes into account both short- and long-range temporal interactions of objects detected by a single camera as well as spatial interactions between cameras in a single optimization problem.
% This allows for a joint reasoning during the data association step across time and different cameras.
% Our model works on either detections or tracklets generated by traditional single camera MOT approaches.
% This allows us to harness the great progress made in single-camera MOT.
% However, crucially, we improve upon single camera MOT by taking into account 3D-information and data association between tracklets observed in different cameras.
% This strictly improves upon what we could obtain from using only trackers for the single camera setting.
\myparagraph{Contributions} Our main contributions can be summarized as follows. First, we introduce a new pre-clustering algorithm driven by 3D geometry projections to group detections at each timestep across cameras. This effectively eliminates tracklet errors from single-camera trackers and provides highly accurate affinity costs for the data association step.
Second, we propose a novel spatial-temporal lifted multicut formulation for the multi-camera setting, jointly optimizing both intra- and inter-camera as well as short- and long-range interaction in a single global formulation.
Finally, we obtain nearly perfect performance on the large-scale WILDTRACK~\cite{chavdarova2018wildtrack} dataset, outperform state-of-the-art on Campus~\cite{xu2016multi} and are on par with the PETS-09~\cite{ellis2009pets2009} dataset. 
% The data association between cameras occurs at three points:
% First, we filter the input tracklets by splitting them up at likely ID-switch positions based on a 3D-clustering pre-processing step.
% Second, data association probabilities are computed for the filtered tracklets based on traditional features from the single camera setting (mainly visual appearance cues) as well as features based on the 3D-information provided by multiple cameras.
% Third, the data association probabilities serve as costs in the final optimization problem.
% Results turn out superior w.r.t.\ the single camera setting because data association is jointly influenced by spatial and temporal information as well as the enforced consistency of tracks for each camera.

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/issues.tex <==
- multi-cut -> multicut (Done!)
- Change much more -> more, remove very unless really needed. In general, do not use superlatives. (Done!)
- In specific -> either Specifically or In particular (Done!)
- Consistent paragraph titles (Capitalization, punctuation) (Done)
- Use tenses consistently (do not switch without reason from present to past and vice versa). (Done)

- Have one big document and use proper references for stuff in the appendix. (Done)

- Update reference given a merge of the main and appendix file.  (Done)


==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/method.tex <==
\begin{figure*}[!hbt]
\centering
\includegraphics[width=1.0\textwidth]{./imgs/Figure_overview_v7.png}
\vspace{-0.3in}
\caption{
Illustration of our LMGP framework.
(a)~Input bounding boxes are given at each camera and each timepoint.
(b)~Bounding boxes observed from different cameras at the same time point are preliminary brought into correspondence through our 3D geometry based pre-clustering step.
(c)~A spatial-temporal tracking graph is constructed.
Nodes in the graph correspond to tracklets generated by a single-camera tracker that are split up at likely ID-switch positions based on features estimated from (b) step via an ID-Error predictor $f_{\mathrm{split}}$.
Edges correspond to possibly associations between tracklets with temporal edges $e^{t}$ (base and lifted for short and long range interaction in the same camera), spatial edges $e^{s}$ (different cameras, overlapping timeframes), and trajectory constraint edges $e^{c}$ (same camera, overlapping timeframes).
(d)~Association costs between nodes are computed between pre-processed tracklets using two networks $f_{\mathrm{temporal}}, f_{\mathrm{spatial}}$ for intra- and inter-camera edges in the tracking graph.
(e)~Tracklets in the tracking graph (c) are clustered together into trajectories via our lifted multicut optimization problem using affinity costs in (d).
(f)~3D coordinates of trajectories from (e) are generated.}
\label{fig:method-overview}
\vspace{-0.1in}
\end{figure*}

\section{Method}
% Illustration of our multi-camera tracking pipeline.
% (a)~Bounding boxes are computed for each camera and each timepoint.
% (b)~Bounding boxes observed from different cameras at the same time point are preliminary brought into correspondence through a pre-clustering.
% (c)~A spatial-temporal tracking graph is constructed.
% Nodes in the graph correspond to parts of tracklets generated by a single-camera tracker that are split up at likely ID-switch positions based on features computed on the pre-clusters.
% Edges correspond to possibly associations between tracklets.
% Temporal edges connect tracklets observed by the same camera at different timepoints.
% Spatial edges connect tracklets observed by different cameras at the same timepoint.
% (d)~Association costs between nodes in the spatial-temporal tracking graphs are computed.
% (e)~Tracklets are clustered together into trajectories via a lifted multicut optimization problem on the spatial-temporal tracking graph.
% (f)~3D coordinates of trajectories from (e) are computed.
Our tracking pipeline is illustrated in Figure~\ref{fig:method-overview}.
Below we describe each of its steps in detail, i.e.,\ pre-clustering for removing ID-switch errors and improving the subsequent affinity cost computation that is utilized in the global lifted multicut problem for computing multi-camera trajectories.

%It is crucial to emphasize that correspondences at each timeframe derived in the pre-clustering step play essential roles in eliminating ID-Switch errors in the initial tracking graph and improving affinity cost efficiency.  
%, which involves four major steps:
%(i)~pre-clustering of detections from different cameras,
%(ii)~spatial-temporal tracking graph construction, 
%(iii)~computing affinity costs among tracklets and 
%(iv)~generating trajectories by solving a lifted multicut clustering problem~\cite{keuper2015efficient}, where each cluster corresponds to a track for a single person across all cameras. 
%In our formulation, step (i) serves as a preprocessing step through which we are able to correct errors made by 2D-trackers. 
%Step (iii) computes highly reliable affinity costs by considering multiple views of the same object.
%Step (iv) takes into account affinities between cameras as well as long-range temporal ones jointly.

% In the first module (i), given a set of detections across cameras at each time-frame, our algorithm will form a corresponding cluster for each target, which covers all its 2D projections at different views. This procedure can be accomplished by utilizing 3D spatial geometry dependencies of detections in the same and different objects and solving a linear assignment based on their 3D coordinates.  In our formulation, step (i) serves as a fundamental component; thereby, we are able to correct precisely errors in graph construction in step (ii) and establish highly reliable affinity costs in step (iii) by querying multiple instances in the same clustering.  To leverage spatial-dependence over a short time, we compose each node in our tracking graph with a 2D tracklet derived from a state-of-the-art 2D Tracker (CenterTrack, Tracktor) in each camera view and applying it for all cameras to define an initial graph. While the 2D tracklet based approach has benefits with a richer hypothesis representation and decreases the global graph's total size significantly, it may suffer from the ID-Switch problem in each node, i.e., detections of distinct objects are grouped into a single node. Fortunately, in our strategy, this obstacle could be addressed efficiently by using derived clustering results in step (i). In particular, each node in an initial graph will be filtered through verifying each pair of detections with additional unoccluded detections at other cameras, yielding a high-quality graph is attained. Given this filtered graph, the space and time hypothesis could be discriminated by using appearance, motion prediction, and 3D space-dependence constraints feature in step (iii). Finally, tracking results over camera views could be discovered automatically through our novel space-time lifted multi-cut optimization; a scheme with capabilities to reconnect each object's fragments in a long-range and recover missing detections due to severe occlusions synchronizing the object's positions through the cameras.

\myparagraph{Notation}
Before describing each part of our approach in detail, we introduce notation used throughout the paper. 
Let $B$ be the set of detections and $B^{t,j}$ the detections at timestep $t$ observed by camera $j$. 
Each detection $b \in B$ is observed by camera $\cam(b)$ and in timeframe $\dettime(b)$.
%
%$\Gamma = \{\Gamma_i: i = 1, ..., K\}$ is the set of tracks, where $K$ is the number of objects appearing in the scene and is determined as part of the optimization process.
%
%Each track $\Gamma_i = \{\tau_i^{j}: j = 1,\ldots,m\}$ consists of a set of 2D  tracklets.
%They are overlapping at time, since there are multiple cameras looking at the same person.
%
Each single camera tracklet $\tau$ consists of a set of bounding boxes at specific timepoints, i.e.\ $\tau = (b^\tau_1, b^{\tau}_2,..., b^{\tau}_{|\tau|})$, where $b^\tau_l$ is the $l$-th detection of trajectory $\tau$.
Tracklets only contain detections from a single camera, i.e.\ $\cam(b^\tau_1) =...= \cam(b^\tau_{|\tau|})$.
We extend the functions $\cam$ and $\dettime$ to tracklets by $\cam(\tau) = \cam(b_1)$ and $\dettime(\tau) = \{\dettime(b_1),\dettime(b_2),\ldots,\dettime(b_{|\tau|})\}$.
Detections of two tracklets that cover the same timepoint are denoted as
\begin{equation}
O(\tau, \tau') = \{(b,b') \in \tau \times \tau' :  \dettime(b) = \dettime(b')\} \, .
\end{equation}
%\croberto{I know you already have quite a low of indices, but since the tracklet is not the same for all tracklets, it should be $\Gamma_i = \{\tau_i^{j}: j = 1,\ldots,m_{i}\}$}
%Paul: I think below 
%For convenience, we use the following sub-indexes to query the bounding box and time frame of $\tau_{i,\,k}^{c_j}$ at frame $k^{th}$: $\tau_{i,\,k}^{c_j} = (b_{i,k}^{c_j}, t_{i,k}^{c_j}),\ \tau_{i,\,k.box}^{c_j} = b_{i,k}^{c_j},\ \tau_{i,\,k.\mathrm{time}}^{c_j} = t_{i,k}^{c_j}$, and $\tau_{i.\mathrm{time}}^{c_j},\, \tau_{i.\mathrm{bbox}}^{c_j}$ to refer a set of timeframe and bounding boxes of $\tau_{i}^{c_j}$ at cam $c_j$. 
%
We denote by $f$ a feature extractor that, given a bounding box $b$, produces an embedding vector $f(b)$ representing its appearance features.
$h$ denotes a map that takes a bounding box and computes the 3D coordinates of the foot point (center of bottom edge) on the ground plane $(z=0)$~\cite{hartley_zisserman_2004} (Section \ref{sec:transformations} Appendix).
%Finally, we utilize $f(x)$ as a feature extractor that transforms a bounding box $x$ to an embedding vector representing for its appearance features and $h(x)$ as a operation that maps a 2D foot point (center of bottom edge) of bounding box $x$ to a 3D position \cite{hartley_zisserman_2004} on a ground plane $(z=0)$.

\subsection{3D Geometry Based Pre-Clustering}
\label{sec:pre-clustering}
The pre-clustering step aims at bringing into correspondence detections of the same object observed by different cameras at each timeframe (Figure \ref{fig:method-overview}-b).
%These clusters give us the possibility to overcome occlusions observed by a single camera.
This enables us to overcome occlusions observed by a single camera.
In particular, if some object is occluded, we will be able to continue tracking the same object at different views (Figure~\ref{fig:teaser_crop}). Unlike prior works \citep{focken2002towards,mittal2002amulti,you2020real} that applied foreground subtraction or fusing image features from multiple cameras, our algorithm exploits 3D geometry constraints of detection projections of the same object. In particular, we project the bottom edge center of each bounding box to obtain its 3D coordinates (ground point) via map $h$.
%We model each detection in 3D by cylinder models~\cite{chavdarova2018wildtrack} centered on the ground plane. The cylinder's height and width is that of an average person.
Two detections observed by different cameras potentially belong to the same person if, after transformation to 3D, the Euclidean distance of the two ground points is less than the diameter of a typical person, which is approximately the human width average (Figure \ref{fig:2Dclustering}-a Appendix).  
%Paul: We do not really need any cylinders. Just ground points and some radius is all is needed.

% The pre-clustering works as follows:
% For each detection $b$, we consider the set of nearby detections 
% $B(b) = \{ b' \in B^{\mathrm{time}(b),\mathrm{cam}(b)} : \mathrm{dist}(h(b'),h(b)) \leq r \}$ observed by camera $\mathrm{cam}(b)$ at timepoint $\mathrm{time}(b)$ with $\mathrm{dist}(,)$ and $r$ are euclidean distance and radius to scan respectively. Likewise, we consider the set of detections $B(b')$ with $\mathrm{time}(b) = \mathrm{time}(b')$ and $\mathrm{cam}(b) \neq \mathrm{cam}(b')$. We then compute a matching between detections in $B(b)$ and $B(b')$ via a linear assignment problem \cite{burkard1999linear} with costs being the Euclidean distance on the 3D space to find a matching between $b$ to a detection $b'' \in B(b')$.

% and vice versa, if $b''$ is matched to $b \in B(b')$, we record that match. We repeat the above procedure for all remaining cameras producing the Pre-Cluster $C_b$. The algorithm is detailed in the Appendix, Algorithm 1.
The pre-clustering works as follows:
for each detection $b$, we consider the set of nearby detections $B^{t,j}(b) = \{b' \in B^{t,j}: \mathrm{dist}(h(b), h(b')) \leq r\}$ observed by the same camera $j = \cam(b)$ at the same timepoint $t = \dettime(b)$ with $\mathrm{dist}(,)$ and $r$ being Euclidean distance and radius to scan respectively. Likewise for camera $j' \neq \cam(b)$, we consider the set of detections $B^{t,j'}(b)$ observed by camera $j'$ close to the 3D-position $h(b)$.
We next compute a matching between detections of $B^{t,j}(b)$ and $B^{t,j'}(b)$ via a linear assignment problem~\cite{burkard1999linear} with costs being the Euclidean distance.
If $b$ is matched to 
a detection $b' \in B^{t,j'}(b)$ through the matching between $B^{t,j}(b)$ and $B^{t,j'}(b)$, and vice versa, if $b'$ is matched to $b \in B^{t,j}(b')$ through another matching between $B^{t,j'}(b')$ and $B^{t,j}(b')$, we record that match as it represents a confident connection. We denote the  resulting cluster for each detection $b$ as $C_b$.
The whole algorithm is detailed in Algorithm \ref{alg:pre-clustering} in the Appendix.

% \subsection{Visible Detections}
\myparagraph {Visible Detection Clustering}
Let $b \in B$ be a detection and $C_b$ be its cluster obtained after pre-clustering.
Since our algorithm uses only geometric coordinates of bounding boxes, the cluster $C_b$ can include both visible and occluded detections (Figure~\ref{fig:split-tracklet}-b).
Let $h_j$ be the 3D camera position of camera $j$ (Equation~\eqref{eq:camera_3D} in Section \ref{sec:transformations} Appendix).
% \begin{equation}
% \begin{split}
%     O_b &= \{b'' \in B^{t,j}: \iou(b'',b) \geq 0.6\} \\
%     x_{b}^* &= \argmin_{x \in O_b} \dist(h(x), h_j) \\
%     %C'_b &= \{b' \in C_b : \abs{O_{b'}} = 1 \text{ or } b' = x_{b'}^*\} \\
%     C'_b &= \{b' \in C_b : b' = x_{b'}^*\}
%     \label{eq:occlusion-filtering}
% \end{split}
% \end{equation}
First, given the detection $b$, we compute a detection $\visible(b)$ nearest to the camera by
\begin{equation}
\label{eq:occlusion-filtering}
\visible(b) = \begin{cases}\argmin_{b'} \dist(h(b'),h_j) \\
\text{s.t. } b' \in B^{\dettime(b),\cam(b)} : \iou(b',b) \geq 0.6\\
%    O_b &= \{b'' \in B^{\dettime(b),\cam(b)}: \iou(b'',b) \geq 0.6\} \\ 
%    b^*(b) &= \argmin_{\overline{b} \in O_b} \{\dist(h(\overline{b}), h_j) \} \\
\end{cases}
\end{equation}
and then use it to refine the pre-cluster to contain only visible detections by
\begin{equation}
\label{eq:visible-detections-cluster}
C'_b = \{b' \in C_b : b' = \visible(b')\}\,.
\end{equation}

% \textcolor{red}{Given these clusters, we can define visible detections (Eq ) used in splitting tracklets or composing novel affinity costs (Eq. 6, 9)}.

%Likewise for camera $j' \neq \cam(b)$, we consider the set of detections $B^{t,j'}(b)$ observed by camera $j'$ close to the 3D-position $h(b)$.
%Now for each camera $j' \neq \cam(b)$, %On these two sets of detections $B_{\textrm{same-cam}}(b)$ and $B_{\textrm{other-cam}}(j',b)$ in two distinct cameras
% We compute a matching between detections in $B(b)$ and $B(b')$ via a linear assignment problem \cite{burkard1999linear} with costs being the Euclidean distance. 
% If $b$ is matched to a detection $b' \in B(b)$, and vice versa, if $b'$ is matched to $b \in B(b')$, we record that match. We repeat the above procedure for all remaining cameras producing the Pre-Cluster $C_b$. The algorithm is detailed in the Appendix, Algorithm 1.
% \croberto{@Duy Is the text ok ?}


%For each pair of cameras $j$ and $j'$ and for detection $b_{i,k}^j$ we define the set of correspondence candidates as those whose 3D-projection is within the radius $r$ of an average person, i.e.\ $\{ b_{i'}^{j'} : d(h(b_i^j), h(b_{i'}^{j'} \leq r\}$.
%Then, a linear assignment problem is solved with costs between candidates being the Euclidean distance of the center point on the ground plane.
%After having computed correspondences between each pair of cameras in the above way, we filter out inconsistent matches introduced by e.g.\ errors in camera calibration and imprecise bounding boxes as follows:
%%Paul: We should possibly rename 2D-projections clustering. At least use the term consistently!
%The clustering step aims at bringing into correspondence detections of the same object observed by different cameras for a single timeframe.
%These clusters give us the possiblity to overcome occlusion observed by a single camera.
%In particular, if some object is occluded, we will be able to continue tracking the same object at different views.
%Our algorithm uses the fact that detections of the same object must align w.r.t.\ their 3D projections and form a cluster in that space, see Figure~\ref{fig:4Dclustering}.
%We model each detection in 3D by cylinder models~\cite{chavdarova2018wildtrack} centered on the ground plane. The cylinder's height and width is that of an average person.
%Two detections observed by different cameras are potentially belonging to the same person if, after transformation to 3D, the Euclidean distance of the entered ground point is lerrthan the diameter of the cylinders.

%This property leads us to compose the following algorithm.
%Given a detection $b_{i,\ k}^{c_j}$ of the object $i^{th}$ at the frame $k$ in camera $c_j$, we open a circle centering at its 3D position $h(b_{i,\ k}^{c_j})$ with a radius $r$.
%We then define a set of 3D position candidates in camera $c_j$ and $c_i$ ($i \neq j$) which located in this circle. In the next step, the correspondences between two cameras $c_i,\, c_j$ could be obtained by solving a linear assignment problem \cite{munkres1957algorithms} with the cost for a pair of points is its 3D distance in the ground space. Theoretically, $b_{i,k}^{c_j}$ could find its matching detection $b_{i,k}^{c_i}$ in camera $c_i$ through described geometry constraint between $h(b_{i,k}^{c_j})$ and $h(b_{i,k}^{c_i})$ (figure \ref{fig:overview}b). Similarly, by repeating this process to the remaining cameras, we could find pairs of matching $b_{i,k}^{c_j} \rightarrow b_{i,k}^{c_x},\ x\in \{1,\, 2..., m\} \setminus j$. However, due to some errors in calibrated cameras and poor bounding boxes, one way connections starting from $b_{i,k}^{c_j}$ are insufficient, we hence verify in reverse direction, i.e for each $b_{i,k}^{c_x}, (x\neq j)$ we check whether $b_{i,k}^{c_j}$ is matched with $b_{i,k}^{c_x}$, if there exists a such condition, we label a connection between $(b_{i,k}^{c_j},\, b_{i,k}^{c_x})$ as a confidence connection and adding it to cluster $C_{i,\,k}$. Finally, given a pair of dections in $C_{i,\,k}$ whose connection has not been established, we associate for it an implicit connection because they share each other a confidence connection through $b_{i,k}^{c_j}$ (figure \ref{fig:2Dclustering}b). 
%The full details to derive all clusters in each timeframe $k$ are summarized in Algorithm 1 in Appendix. To the best of our knowledge, we are the first team address this problem in the sense of 3D geometry constraints. In the next step, we will highlight how could we leverage this step to pre-processing our tracking graph and establish good similarity for the space-time hypothesis.  
% \begin{figure}[!hbt]
% \centering
% \includegraphics[width=0.5\textwidth]{Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/imgs/2D_Projections_Clustering.png}
% \caption{(a) 3D geometry constrains of points belong to the same object, (b) An illustration of our pre-clustering in WILDTRACK with 7 cameras.}
% \label{fig:2Dclustering}
% \end{figure}

\subsection{Spatial-Temporal Tracking Graph}
\label{sec:spatial-temporal-tracking-graph}
%Paul: Use spatio-temporal or spatial-temporal, but consistently!
We formulate a global spatial-temporal tracking graph $G = (V, E)$, where each node $v \in V$ corresponds to a tracklet $\tau$ in a single camera and edges represent data associations between tracklets across space and time (Figure \ref{fig:method-overview}-c).
A trajectory output will correspond to a cluster of nodes in the tracking graph $G$.
To benefit from current advances in single-camera MOT, each node (tracklet) at each camera is derived from a state-of-the-art tracker.
We use CenterTrack~\cite{zhou2020tracking} in our experiments, but it can be replaced by other trackers.

While recent works \cite{xu2017cross,lan2020semi,he2020multi} directly compute affinity costs and solve the data association on the graph with nodes generated by single-camera trackers, we further correct ID-Switch errors in tracklet proposals (Figure~\ref{fig:split-tracklet}-a).
The ID switches in the original tracklets severely harm the total performance, especially in crowded or cluttered scenes.
To this end, we leverage bounding box correspondences from the pre-clustering and conduct the following steps.

% The original tracklets will be broken up at likely ID-switch positions, which are detected by considering inter-camera associations computed during a pre-clustering step.
% Each obtained sub-tracklet corresponds to a node in $V$.
% Edges $E$ will handle associations between sub-tracklets observed by the same camera at different timepoints (temporal edges $E^{t}$) and between tracklets observed by different cameras but at the same timepoint (spatial edges $E^s$).
% Due to both spatial and temporal edges, each camera view contributes to the final track.
% Thereby, occlusion does not force a track to be discontinued, since the remaining cameras for which the object is still visible can contribute towards a continuation of the track.

% \subsection{Visible Detections}
% \myparagraph {Visible Detections}
% Let $b \in B$ be a detection and $C_b$ its cluster obtained after pre-clustering.
% Since our algorithm uses only geometry coordinates of bounding boxes, the cluster $C_b$ can include both visible and occluded detections (Figure~\ref{fig:split-tracklet}-b).
% Let $h_j$ be the 3D camera position of camera $j$ (Equation~\eqref{eq:camera_3D} in Section \ref{sec:transformations} Appendix).
% % \begin{equation}
% % \begin{split}
% %     O_b &= \{b'' \in B^{t,j}: \iou(b'',b) \geq 0.6\} \\
% %     x_{b}^* &= \argmin_{x \in O_b} \dist(h(x), h_j) \\
% %     %C'_b &= \{b' \in C_b : \abs{O_{b'}} = 1 \text{ or } b' = x_{b'}^*\} \\
% %     C'_b &= \{b' \in C_b : b' = x_{b'}^*\}
% %     \label{eq:occlusion-filtering}
% % \end{split}
% % \end{equation}
% First, given the detection $b$ we compute a detection $\visible(b)$ nearest to the camera by
% \begin{equation}
% \label{eq:occlusion-filtering}
% \visible(b) = \begin{cases}\argmin_{b'} \dist(h(b'),h_j) \\
% \text{s.t. } b' \in B^{\dettime(b),\cam(b)} : \iou(b',b) \geq 0.6\\
% %    O_b &= \{b'' \in B^{\dettime(b),\cam(b)}: \iou(b'',b) \geq 0.6\} \\ 
% %    b^*(b) &= \argmin_{\overline{b} \in O_b} \{\dist(h(\overline{b}), h_j) \} \\
% \end{cases}
% \end{equation}
% and then use it to refine the pre-cluster to contain only visible detections by
% \begin{equation}
% C'_b = \{b' \in C_b : b' = \visible(b')\}\,.
% \end{equation}
%In words, $C'_b$ contains only those detections that are nearest to the camera or $C_b$ if there are no other detections nearby.

%\begin{equation*}
%\resizebox{.4 \textwidth}{!} { $
%C^{'}_{i,k} = \{b_{i,k}^{c_j} \in C_{i,k}: \ |O(b_{i,k}^{c_j})| = 0 \textrm{ or } b_{i,k}^{c_j} = x^{*}\}
%$}
%\end{equation*}
%where $x^{*} = \argmin_{x \in O(b_{i,k}^{c_j})}||h(x) - h(c_j)||^2$, $O_{i,k}^{c_j} = \{x: \textrm{iou}(x, b_{i,k}^{c_j}) \geq 0.6\}$, \textrm{iou} indicates for intersection over union overlapping metric \cite{szeliski2010computer}, and $h(c_j)$ is a transformation that computes the 3D coordinate of camera center point $c_j$. The above equation is combined between $\textrm{iou}$ metric in the 2D image coordinate and consistent in 3D space to avoid ambiguity; thereby, given the same overlapping score, we could not know precisely whether a target detection is occluded or not.
% \croberto{ (1) It should be $C_{b} \setminus \{b\}$, as the cluster depends on $b$. (3) $x^{*}$ is optimized over all detections in $O_{b'}$, so I would denote it something like $x(b)^{*}$. 
% (4) If I take a detection  $b$ at time $t$ from camera $j$, then I get a detection $b' \in C \setminus \{b \}$ that corresponds to the same person, but from another camera $j'$ at time $t$. Then $O_{b'}$ collects all detections at camera $j'$ at time $t$ with big overlap. In particular $b' \in O_{b'}$ and thus $|O_{b'}| \geq 1$.  
% (5)
% If $b' = x^{*}$, then $b'$ is nearest to camera $j'$, compared to all detections $b'' \in O_{b'}$ that have a big overlap with $b'$?}

\myparagraph{Feature Extension on Detection Clusters}
Given a pair of detections $b, b' \in B$ at different timepoints of potentially the same object and an embedding feature $f$ (we use DG-Net~\cite{zheng2019joint}), we aim to obtain robust association features by considering relations between detections in the visible cluster $C_{b}^{'}$ (Equation \ref{eq:visible-detections-cluster}). To this end, we first compute for all pairs of detections in $(\bar b, \bar b') \in C'_b \times C'_{b'}$ their cosine similarity w.r.t.\ features extracted by $f$, that is
$D_{\bar b, \bar b'} = \langle f(\bar b), f(\bar b') \rangle$.
Next, we solve a linear assignment problem between $C'_b$ and $C'_{b'}$ with costs $D_{\bar b, \bar b'}$ for each pair $(\bar b, \bar b') \in C'_b \times C'_{b'}$.
Let the set of matches be $M = \{(\bar b, \bar b') \in C'_b \times C'_{b'}: \bar b \text{ and } \bar b' \text{ are matched}\}$.
On the matches we estimate the following statistical similarities:
\begin{multline}
   c_{b,b'}^{\mathrm{best}} = \min_{(\bar b, \bar b') \in C'_b \times C'_{b'}} D_{\bar b, \bar b'}, \quad
   c_{b,b'}^{\mathrm{min}} = \min_{(\bar b, \bar b') \in M} D_{\bar b, \bar b'}, \\
   c_{b,b'}^{\mathrm{max}} = \max_{(\bar b, \bar b') \in M} D_{\bar b, \bar b'}, \quad
   c_{b,b'}^{\mathrm{mean}} = \frac{\sum_{(\bar b, \bar b') \in M} D_{\bar b, \bar b'}}{\abs{M}}, \\
   c_{b,b'}^{\mathrm{var}} = \sum_{(\bar b, \bar b') \in M} (D_{\bar b, \bar b'} - c_{b,b'}^{\mathrm{mean}})^2 \,.
   \label{eq:detection-cluster-features}
\end{multline}
\myparagraph{Splitting Tracklets}
\label{subsec:split-tracklets}
We now construct a network $f_{\mathrm{split}}$ (see Appendix \ref{appendix:network_architecture} for the architecture details) for correcting ID-Switch errors. Specifically, for each tracklet $\tau$,  $f_{\mathrm{split}}$
scans over all consecutive detections $(b,b') \subset \tau$ (Figure \ref{fig:split-tracklet}-a), takes their respective similarity values from Equations \ref{eq:detection-cluster-features} using the visible detections $C_{b}^{'},\, C_{b'}^{'}$ (Figure \ref{fig:split-tracklet}-b) and returns a probability score indicating whether or not they belong to the same tracklet.
$\tau$ is split into sub-tracklets at the predicted ID-switch error positions that become new nodes in our spatial-temporal tracking graph (Figure \ref{fig:split-tracklet}-c). 
% We use $f_{\mathrm{split}}$ on consecutive detections of the initial tracklets generated by the single camera trackers and split them whenever $f_{\mathrm{split}}$ indicates so.
% We choose the embedding feature $f$ to be DG-Net~\cite{zheng2019joint}, a state of the art deep network for re-identification.
% Each sub-tracklet becomes a node $V$ in the spatial-temporal tracking graph.
\begin{figure}[!hbt]
\centering
\includegraphics[width=0.5\textwidth]{./imgs/Split_Tracklet.png}
\vspace{-0.3in}
\caption{(a) A tracklet (node) $\tau$ with ID-Switch error (two red dashed rectangles) in an initial tracking graph, (b) Using visible clusters of  detections at two consecutive frames, we can cut at the error positions, (c) Two new sub-tracklets $\tau',\, \tau''$  of distinct objects are generated.}
\label{fig:split-tracklet}
\end{figure}

%Given above features, we could learn a network $f_{\mathrm{filter}}$, which will scan and cut for each node $v\in V$ into $m + 1$ sub nodes $v_{f}$ if $v$ includes $m$ ID-Switch positions, i.e., mixing detections of distinct objects into a single one. In short, finishing step will create a new filtered graph $G_{f} = (V_{f}, E')$ where each node $v_{f} \in V_{f}$ has been eliminated with ID-switch noises \cite{leal2015motchallenge,milan2016mot16}. An visualizing figure for this step is illustrated in the appendix.

\subsection{Learning Affinities with Multi-Camera Setting}
\label{sec:affinity-costs}
Given the tracking graph $G = (V, E)$ after pre-processing for ID-Switch error removal, we compute for pairs of tracklets $\tau=(b_1,\ldots,b_{\abs{\tau}})$ and $\tau' = (b'_1,\ldots,b'_{\abs{\tau'}})$ affinities representing the probability that both $\tau$ and $\tau'$ track the same object.
To this end, we consider standard cues based on motion information as in~\cite{9242263,xu2017cross,wen2017multi}.
We additionally propose novel appearance and 3D position-based similarity costs which harness image correspondences from our 3D pre-clustering step.
% Given two tracklets $\tau=(b_1,\ldots,b_{\abs{\tau}})$ and $\tau' = (b'_1,\ldots,b'_{\abs{\tau'}})$, we compute the affinity representing the probability that both $\tau$ and $\tau'$ track the same object.
% To this end, we consider cues such as appearance and motion information~\cite{9242263,xu2017cross,wen2017multi} as well as a novel 3D position based similarity cost.
\vspace{-0.1in}
\subsubsection{Temporal Affinites }
\label{sec:temporal-edge-affinities}
Let $\tau$ and $\tau'$ be two tracklets, observed by the same camera and with $\dettime(b_{\abs{\tau}}) < \dettime(b'_1)$, i.e.\ following each other temporally.
We compute their similarity based on  motion and appearance.

\myparagraph{Forward/Backward Motion Affinities}
Motion extrapolation of $\tau$ to subsequent or extrapolation of $\tau'$ to previous timeframes can provide evidence of whether the two tracklets belong to the same object.
We adopt features from~\cite{xu2017cross,wen2017multi} for our settings by using the first/last $m$ frames from each tracklet to estimate an average velocity and then predict the forward velocity $\vec{v}_{\tau}$ of $\tau$ and the backward velocity $\overleftarrow{v}_{\tau'}$ of $\tau'$. The forward $c^{\mathrm{fw,t}}$ and backward $c^{\mathrm{bw,t}}$ affinity are computed by:
\begin{equation}
\label{eq:temporal-forward-backward-affinity-cost}
\begin{split}
 c^{\mathrm{fw,t}}(\tau, \tau') & =  \norm{h(b_{\abs{\tau}}) + \text{disp}(\tau,\tau') - h(b'_1)} \,.\\
c^{\mathrm{bw,t}}(\tau, \tau') & =  \norm{h(b'_{1}) - \text{disp}(\tau,\tau') - h(b_{\abs{\tau}})}  \,.
\end{split}
\end{equation}
where $\text{disp}(\tau,\tau') = \vec{v}_{\tau} \cdot t(\tau, \tau');\, t(\tau, \tau') = (\dettime(b'_1) - \dettime(b_{\abs{\tau}}))$. 

% The forward temporal affinity $c^{\mathrm{fw,t}}$ is
% \begin{equation}
% \label{eq:temporal-forward-affinity-cost}
% \begin{split}
% t(\tau, \tau') &= (\dettime(b'_1) - \dettime(b_{\abs{\tau}}))\\
% \overrightarrow{\text{disp}}(\tau,\tau') & = \vec{v}_{\tau} \cdot t(\tau, \tau') \\
%   c^{\mathrm{fw,t}}(\tau, \tau') & =  \norm{h(b_{\abs{\tau}}) + \overrightarrow{\text{disp}}(\tau,\tau') - h(b'_1)} \,.
%   \end{split}
% \end{equation}
% The backward temporal affinity $c^{\mathrm{bw,t}}$ is
% \begin{equation}
% \begin{split}
% \label{eq:temporal-backward-affinity-cost}
% \overleftarrow{\text{disp}}(\tau,\tau') & = - \overleftarrow{v}_{\tau'} \cdot t(\tau, \tau')  \\ 
%   c^{\mathrm{bw,t}}(\tau, \tau') & =  \norm{h(b'_{1}) + \overleftarrow{\text{disp}}(\tau,\tau') - h(b_{\abs{\tau}})}  \,.
%   \end{split}
% \end{equation}

%Paul: this should go into lifted multicut section.
%which connects two nodes (two tracklets) $(\tau_{x}^{c_j}, \, \tau_{y}^{c_j})$ at camera $c_j$, we only assign a cost for it if the distance in time $c_{e^{\mathrm{time}}}^{\mathrm{time}}$ is less than or equal $10$ seconds. Along with it, if $c_{e^{\mathrm{time}}}^{\mathrm{time}} \geq 5$ seconds, we label it as lifted-edges where $c_{e^{\mathrm{time}}}^{\mathrm{time}} = |\tau_{x,\, \mathrm{last}.\mathrm{time}}^{c_j} - \tau_{y,\, \mathrm{first}.\mathrm{time}}^{c_j}| $
\myparagraph{Multi-view Appearance Affinities}
Tracklets belonging to the same object should share a similar appearance across time and cameras.
We measure this by computing
\begin{equation}
\label{eq:appearance-affinity}
        c^{\mathrm{app}}_{\mathrm{index}} (\tau, \tau') = \sum_{b \in \tau}\sum_{b' \in \tau'}  \frac{c_{\mathrm{index}}^{b,b'}}{\abs{\tau}\abs{\tau'}} \, , 
\end{equation}
where $\mathrm{index} \in \{\mathrm{best,min,max,mean,std}\}$ and each score $c_{\mathrm{index}}(b,b')$ is computed as in Equation \ref{eq:detection-cluster-features}. Note that we associate each detection with its visible image correspondences derived from the pre-clustering step in Equations \ref{eq:occlusion-filtering}, which sets us apart from prior works \cite{9242263,wen2017multi,lan2020semi} as both intra- and inter-camera information can be associated simultaneously.
% which enables us to exploit both intra- and inter-camera information simultaneously. This point thus sets us apart from prior works \cite{9242263,wen2017multi,lan2020semi}.
An ablation study showing the benefit of this new cost can be found in Table \ref{tab:temporal-costs-performance} Appendix.
\vspace{-0.1in}
\subsubsection{Spatial Affinities}
\label{sec:spatial-edge-affinities}
For each pair of tracklets $\tau$ and $\tau'$ observed by different cameras and overlapping in time, we compute affinities based on similarity of motion and average 3D distance of their projected detections as in~\cite{xu2017cross,wen2017multi}.
We additionally propose  novel pre-clustering agreement based-similarity scores for each timestep on which they overlap.

% For each pair of tracklets $\tau$ and $\tau'$ with $\cam(\tau) \neq \cam(\tau')$ and $\dettime(\tau) \cap \dettime(\tau') \neq \varnothing$, \ie tracklets observed by different cameras overlapping in time, we compute several affinities based on similarity of motion, average 3D distance of their projected detections, and their pre-cluster similarity for each timestep on which they overlap.

%$e^{\mathrm{space}} \in E^{\mathrm{space}}$ that links a pair of tracklets $(\tau_{x}^{c_i}, \, \tau_{y}^{c_j}), i \neq j$, an associated aff will be computed if they are overlap in time and there exists at least an overlap time frame so that the 3D distance between $\tau_{x}^{c_i}$ and $\tau_{y}^{c_j}$  is less than or equal a radius of $r$, i.e., $\tau_{x.\mathrm{time}}^{c_i} \cap \tau_{y.\mathrm{time}}^{c_j} = O_{x, y}$ then $O_{xy}  \neq \emptyset$ and $\exists k \in O_{xy}: ||h(\tau_{y, k.\mathrm{bbox}}) - h(\tau_{x, k.\mathrm{bbox}})|| \leq r$

\myparagraph{Forward/Backward Motion Affinities}
Similar to temporal forward resp.\ backward affinities, we will also exploit motion information in the spatial setting.
If, for example $\max\{\dettime(\tau)\} < \max\{\dettime(\tau')\}$,
we let $\vec{v}_{\tau}$ be the forward velocity of $\tau$.
The spatial forward affinity is defined as
\begin{equation}
    \label{eq:spatial-forward-affinity}
    c^{\mathrm{fw,s}}(\tau, \tau') = \norm{h(b_{\abs{\tau}}) + \vec{v}_{\tau} - h(b'_{\abs{\tau}+1})} \,.
\end{equation}
The spatial backward affinity $c^{bw,t}$ is defined analoguously.

%Likely time-edges, we could also use this feature to measure the deviation between each object's moving paths at different camera views. Without loss of generality, we can assume $|\tau_{x.\mathrm{time}}^{c_i}| > |\tau_{y.\mathrm{time}}^{c_j}|$, forward cost could be estimated by:
%\begin{equation*}
%\resizebox{0.95\linewidth}{!}{$
%   c_{e^{\mathrm{space}}}^{fw}(\tau_{x}^{c_i}, \, \tau_{y}^{c_j}) =  ||h(\tau_{y,\,\mathrm{last}.\mathrm{bbox}}^{c_j}) + \vec{v}_{\tau_y} - h(\tau_{x,\,(\mathrm{last} + 1).\mathrm{bbox}}^{c_i})||
%   $}
%\end{equation*}
%where $\vec{v}_{\tau_y}$ is an estimated averaged velocity of $\tau_y$. Similar, we could also define for the backward cost.
%\vspace{-0.1in}

\myparagraph{Average 3D Distance Affinity}
Given two tracklets of the same object, the bounding boxes at timepoints covered by both should have a small distance w.r.t.\ 3D projections.
We capture this property by defining the average 3D distance affinity as
\begin{equation}
\label{eq:average-3d-distance-affinity}
     c^{\mathrm{avg 3D}}(\tau, \tau') = \sum_{(b,b') \in O (\tau, \tau')}
    \frac{\norm{h(b) - h(b')}}{
   \abs{O(\tau,\tau')} 
    }\,.
\end{equation}

\myparagraph{Pre-clustering Agreement Affinity}
The pre-clustering of two tracklets of the same object on shared timesteps should coincide. We define a novel metric to quantify this by

% Given two tracklets, their pre-clustering on shared timesteps should coincide.
% We define a corresponding affinity as
\begin{equation}
\label{eq:pre-clustering-affinity}
c^{\mathrm{pc}}(\tau,\tau') = 
\sum_{(b,b') \in O(\tau,\tau')} \frac{p \cdot \mathbbmss{1}_{[C_b = C_{b'}]} + (1-p)\mathbbmss{1}_{[C_b \neq C_{b'}]} }{\abs{O(\tau,\tau')}} 
\end{equation}
for some prior probability $p$ (we choose $0.8$). 
The contributions of Equation \eqref{eq:pre-clustering-affinity} in capturing similarity among spatial tracklets can be seen in Table~\ref{tab:spatial-costs-performance} Appendix.
% We present ablation studies showing contributions of~\eqref{eq:pre-clustering-affinity} in capturing similarity among tracklets in Table \ref{tab:spatial-costs-performance} Appendix.

%\subsubsection{Learning Spatial-Temporal Affinity}
%\label{sub:learninig-spatial}
%Given described features, we could learn two networks $f_{\mathrm{space}}$ and $f_{\mathrm{time}}$ to return an affinity cost for space and time edges correspondingly. Specially,
% \resizebox{1.0\linewidth}{!}{
% \begin{minipage}{\linewidth}
% \begin{align*}
%       &\hspace{0.15in}c_{e^{\mathrm{space}}}(e) = \log \left(\frac{p_e}{1-p_e}\right),\ p_e = f_{\mathrm{space}}(e),\ e \in E^{\mathrm{space}} \\
% &\hspace{0.15in}c_{e^{\mathrm{time}}}(e) = \log\left(\frac{p_e}{1-p_e}\right),\ p_e = f_{\mathrm{time}}(e),\ e \in E^{\mathrm{time}} 
% \end{align*}
% \vspace{0.005in}
% \end{minipage}}
% \resizebox{1.0\linewidth}{!}{
% \begin{minipage}{\linewidth}
% \begin{align*}
%       &\hspace{0.15in}c_{e^{t}}(e) = \log \left(\frac{p_e}{1-p_e}\right),\ p_e = f_{t}(e),\ e \in E^{t}\
% \end{align*}
% \vspace{0.01in}
% \end{minipage}}
% \begin{equation*}
% c_{e^{t}}(e) = \log \left(\frac{p_e}{1-p_e}\right),\ p_e = f_{t}(e),\ e \in E^{t}\
% \end{equation*}
%$c_{e^{t}}(e) = \log \left(\frac{p_e}{1-p_e}\right)$ with $p_e = f_{t}(e),\ e \in E^{t},\, t \in \{\mathrm{space}, \mathrm{time}\}$. Since our graph uses each node as a tracklet whose length varies depending on the camera, therefore, it is not straightforward to pair samples of the same and different objects during the training step. We hence propose a sampling strategy over spatial-temporal possible edges to capture complex situations that could happen during the testing procedure. These algorithms are presented in Appendix.

\subsection{Lifted Multicut for Multi-Camera Tracking}
\label{sec:lifted-multicut-optimization}
We first recapitulate the lifted multicut problem and use it to formulate the multi-camera MOT problem.
Our formulation extends the (lifted-) multicut works for single-camera MOT~\cite{tang2015subgraph,tang2016multi,tang2017multiple} to multiple cameras.

\myparagraph{Lifted Multicut} 
The multicut optimization problem~\cite{chopra1993partition} is to partition nodes of a given graph $G=(V,E)$ with edge weights $c: E \rightarrow \R$ into a number of clusters $\Pi = (\Pi_1,\ldots,\Pi_k)$, where the number of clusters $k$ is determined as part of the optimization problem.
The clusters form a partition of $V$, i.e.\ $\Pi_i \cap \Pi_j = \varnothing$ $\for i \neq j$ and $\Pi_1 \cup \ldots \cup \Pi_k = V$ where each component $\Pi_i  \in \Pi$ implies a connected subgraph of $G$.
A multicut is an edge indicator vector $y: {E} \rightarrow \{0,1\}$ defined  by $y_e = 0$ iff the endpoints of $e$ are in the same component. 
The multicut problem can be written as an integer linear program:
\begin{equation}
        \min_{y \in \{0,\,1\}^{E}} \sum_{e \in E}c_{e}\,y_{e}
\end{equation}
\vspace{-0.1in}
\begin{equation}
\label{eq:multi-cut-constraint}
        \mathrm{s.t.\ } \forall C \in \mathrm{cycles}(G),\ \forall e \in C: y_{e} \leq \sum_{\bar{e} \in C  \setminus \{e\}}\, y_{\bar{e}}.
\end{equation}

The lifted multicut problem~\cite{keuper2015lifted} augments the original multicut problem by introducting a second set of lifted edges $E'$ together with lifted edge costs $c' : E' \rightarrow \R$.
% Lifted edges serve as connectivity priors for their endpoints w.r.t.\ to a partition and the base edges $E$.
For any edge $e' = (i,j) \in E'$ and clusters $(\Pi_1,\ldots,\Pi_k)$, a lifted edge indicator vector is defined as
\begin{equation}
\label{eq:lifted_constraints}
    \hspace{-0.15in}y_{e'} = 0 \Leftrightarrow \exists l \text{ and a path }P 
    \in ij\text{-paths}(G)
    \text{ s.t. } P \in \Pi_l.\hspace{-0.1in}
\end{equation}
% \vspace{-0.25in}
% \begin{multline}
%     \label{eq:def_path}
%      \hspace{-0.15in} \text{where }ij \text{-paths}(G) = \big\{(v_{1},v_{2},...,v_{l-1},v_{l}): (v_{i}v_{i+1}) \in E,\\ \, v_{1} = i,\, v_{l} = j \big\}
% \end{multline}
In words, the label of lifted edge is $0$ iff there exists a path connecting its endpoints through base edges in $E$ and through nodes that all are in a single cluster.
% Lifted edges are connectivity priors for their endpoints w.r.t.\ to a partition and the normal edges $E$.
% Given a partition $(\Pi_1,\ldots,\Pi_k)$, a lifted edge indicator vector is defined as
% \begin{equation}
% y'^{\Pi}_{ij} = 1 \Leftrightarrow \exists l \text{ and } ij\text{-path } P \text{ in } G \text{ s.t. } P \in \Pi_l\,.
% \end{equation}
% In words, a lifted edge is active iff there is a path connecting its endpoints through normal edges in $E$ and visiting nodes of a single cluster only.

\myparagraph{Spatial-Temporal Lifted Tracking Graph} We now propose our lifted multicut for multiple object tracking given a spatial-temporal graph. Specifically, three types of edges are employed: temporal, spatial, and constraint edges (Figure \ref{fig:method-overview}-c). The temporal edges $E^{t}_{t_{\mathrm{max}}}$ connect tracklet nodes observed by the same camera at different timesteps up to some maximal time threshold $t_{\mathrm{max}}$ (10 seconds in our experiments), spatial edges $E^{s}$ connect tracklets observed by different cameras at overlapping timeframes, and tracklet nodes that are observed by the same camera and have overlapping timeframes are forbidden to end up in the same trajectory through constraint edges $E^c$. The formulations for these edge sets are:
\begin{equation}
\resizebox{.5 \textwidth}{!}{$
    \begin{split}
        E^{t}_{t_{\mathrm{max}}} & = \left\{ (\tau,\tau') :
        \begin{array}{c}
        \cam(\tau) = \cam(\tau'), \\
         \max\{\dettime(\tau')\} - \min\{\dettime(\tau)\} \in (0, t_{max}]
        \end{array}
        \right\} \\
        E^{s} & = \left\{ (\tau,\tau') : 
        \begin{array}{c}\cam(\tau) \neq \cam(\tau'), \\
        \dettime(\tau) \cap \dettime(\tau') \neq \varnothing
        \end{array}
        \right\}\\
        E^c &= \left\{ (\tau, \tau') \in V \times V:
        \begin{array}{c}
        \cam(\tau) = \cam(\tau'), \\
        \dettime(\tau) \cap \dettime(\tau') \neq \varnothing 
        \end{array}
        \right\}\,. 
    \end{split}$}
\end{equation}
% \begin{equation}
% E^c = \left\{ (\tau, \tau') \in V \times V:
% \begin{array}{c}
% \cam(\tau) = \cam(\tau'), \\
% \dettime(\tau) \cap \dettime(\tau') \neq \varnothing 
% \end{array}
% \right\}\,. 
% \end{equation} 
%Here edges in $E^c$ will be utilized as soft restrictions to enforce that  a cluster does not cover two detections in the same timeframe observed by the same camera, i.e. of two distinct objects.
Given the above edges, we divide them into 
base edges $E$ and lifted edges $E'$:
\begin{equation}
    E = E^{t}_{\mathrm{5sec}}  \cup E^c \cup E^s;
    E' = E^{t}_{\mathrm{10sec}} \backslash E^t_{\mathrm{5sec}}\,.
\end{equation}
That is, all edges such that tracklets have temporal distance less than $5$ seconds are base edges ($e^{t}_{\mathrm{base}}$), while temporal edges with larger time distance $t_{\mathrm{max}}$ are lifted ones ($e^{t}_{\mathrm{lift}}$).
The lifted edges are used here to incorporate long-range interactions of objects, i.e.\ handling the case when an object disappears due to occlusion and reappears again.

The edge costs $c_{e^{t}}$ and $ c_{e^{s}}$ for temporal $e^{t} \in E^{t}_{\mathrm{t_{max}}}$ and spatial edges $e^{s} \in E^{s}$ in our framework are produced by two neural networks $f_{\mathrm{temporal}}$ and $f_{\mathrm{spatial}}$, which take input features described in Section \ref{sec:affinity-costs} and return a similarity score (Subsection \ref{sec:computing-affinity} Appendix). 
We also assign a large negative value $c_{e^{c}} = M \ll 0$ for each $e^{c} \in E^c$ to guarantee that clusters are trajectories. 

% Our formulation as lifted multicut has been introduced for single camera MOT in~\cite{tang2017multiple}.
% The lifted edges force the clusters to be temporally consistent.
% A time gap between tracklets in a trajectory that is too large will force some intermediate tracklet to be selected through the connectivity prior introduced by the corresponding lifted edge.


% \myparagraph{Edge Costs for Spatial-Temporal Lifted Graph} For each type of edge, we have to assign for it a corresponding edge cost, representing the correlation between the two tracklets. We compute edge costs $c^t$ for temporal edges $e^{t} = (\tau, \tau') \in E^{t}_{\mathrm{10sec}}$ from the affinities described in Section~\ref{sec:temporal-edge-affinities}.
% In particular,
% \begin{multline}
% c_{e^{t}} = f_{\mathrm{temporal}}(c_{\mathrm{index}}^{\mathrm{app}}(\tau,\tau'), c^{\mathrm{fw,t}}(\tau,\tau'),\\ c^{\mathrm{bw,t}}(\tau,\tau'),\, t(\tau, \tau')),
% \end{multline}
% where $\mathrm{index} \in \{\mathrm{best,min,max,avg,std}\}$,\,$f_{\mathrm{temporal}}$ is a neural network,  and the affinities are from~\eqref{eq:appearance-affinity},~\eqref{eq:temporal-forward-affinity-cost} and~\eqref{eq:temporal-backward-affinity-cost}. Similarly, spatial edge cost for $e^{s} = (\tau, \tau') \in E^{s}$ is computed by
% \begin{multline}
%     c_{e^{s}} = f_{\mathrm{spatial}}(c^{\mathrm{fw,s}}(\tau,\tau'), c^{\mathrm{bw,s}}(\tau,\tau'),\\ c^{\mathrm{avg 3D}}(\tau,\tau'), c^{\mathrm{pc}}(\tau,\tau'))
% \end{multline}
% with $f_{\mathrm{spatial}}$ is another neural network and affinities are from~~\eqref{eq:spatial-forward-affinity},~\eqref{eq:average-3d-distance-affinity} and~\eqref{eq:pre-clustering-affinity}.
% Training details and the accuracy of these local costs are presented in the Appendix. To enforce that clusters are trajectories, we also assign a large negative value $c_{e^{c}} = M \ll 0$ for each $e^{c} \in E^c$. 

% Paul: Just remove (or just keep the solver part.)

\myparagraph{Lifted Multicut Formulation}
We state our lifted multicut optimization for the multi-camera tracking as: 
\begin{equation}
\begin{gathered}
    \min\limits_{y \in \{0,1\}^{E \cup E'}}  \sum\limits_{e^{t} \in E^{t}_{t_{\mathrm{max}}}}c_{e^{t}}\,y_{e^{t}} + \sum\limits_{e^{s} \in E^{s}}c_{e^{s}}\,y_{e^{s}} + \sum\limits_{e^{c} \in E^{c}}M\,y_{e^{c}}\\
    \text{s.t. }  y \text{ obeys Equations }\eqref{eq:multi-cut-constraint} \text{ and }\eqref{eq:lifted_constraints}.
    \end{gathered}
    \label{eq:proposed-lmp}
\end{equation}
Since this formulation is NP-Hard \cite{keuper2015lifted}, we resort to efficient heuristic solvers presented in Section \ref{sec:solver-lmp} Appendix.


%\myparagraph{Objective Function.} 
%We state our lifted multi-cut optimization for the %multi-camera tracking is: 
%\begin{equation}
%\label{eq:lifted-multicut}
%    \small{\hspace{-0.1in}\min_{(y) \in \{0,1\}^{E \cup E'}}\sum_{e^{t} \in E^{t}}c_{e^{t}}\,y_{e^{t}} + \sum_{e^{s} \in E^{s}}c_{e^{s}}\,y_{e^{s}} + \sum_{e^{c} \in E^{c}}M\,y_{e^{c}}}
%\end{equation}
%\begin{equation}
%   \small{\mathrm{s.t.\ } \forall C \in \mathrm{cycles}(G),\ \forall e \in C: y_{e} \leq \sum_{f \in C  \setminus \{e\}}y_{f}}
%\end{equation}
%\begin{equation}
%    \small{\forall e'=(\tau,\tau') \in E',\,  \forall P \in \tau\tau' \textrm{-paths}(G):y_{e'} \leq \sum_{f \in P} y_{f} \label{eq:lift-path}}
%\end{equation}
%\begin{equation}
%    \small{\forall e' = (\tau,\tau') \in E',\, \forall C \in \tau\tau' \textrm{-cuts}(G) : 1 - y_{e'} \leq \sum_{f \in C} (1-y_{f}) \label{eq:lift-cut}}
%\end{equation}
%where $\tau\tau' \textrm{-cuts}(G)$ is any cut in $G$ assigning $\tau$ and $\tau'$ to different groups, the $\textrm{cycles}(G)$ denotes the set of cycles in graph $G$, and $\tau\tau' \textrm{-paths}(G)$ is the set of paths in $G$ connecting $\tau$ and $\tau'$ . The equations \ref{eq:lift-path} and \ref{eq:lift-cut} are equivalent to the lifted path constraint in Equation \ref{eq:lifted_constraints} but adapted in our tracking graph. We present a  solver for this problem in Section 5, Appendix.

% \begin{equation}
%     \min_{(y^t,y^s,y^r) \in \{0,1\}^{\abs{E^t} + \abs{E^s} + \abs{E^r}}}
%   \langle c^t, y^t \rangle +  
%   \langle c^s, y^s \rangle +  
%   \langle M, y^r \rangle\,.
% \end{equation}



%To obtain tracking results on the filter graph $G_{f} = (V_{f}, E'),\, E' = E^{\mathrm{time}} \cup E^{\mathrm{space}},\, E^{\mathrm{time}} = E_{\mathrm{reg}}^{\mathrm{time}} \cup E_{\mathrm{\mathrm{lift}}}^{\mathrm{time}}$ with designed affinity costs $c_{e^{\mathrm{space}}},\, c_{e^{\mathrm{time}}}$, we propose a novel space-time lifted cut optimization: 
%\resizebox{0.9\linewidth}{!}{
%\begin{minipage}{\linewidth}
%\begin{multline*}
%\min_{y \in \{0, \,1\}^{E'}} \sum_{e^{\mathrm{space}} \in E^{\mathrm{space}}} c_{e^{\mathrm{space}}}\,y_{e^{\mathrm{space}}} + \sum_{e^{\mathrm{time}} \in E^{\mathrm{time}}} c_{e^{\mathrm{time}}}\,y_{e^{\mathrm{time}}}\\
%\textrm{subject to } \forall C \in \textrm{cycles}(G_{f}) , \forall e 
%\in C: y_e \leq \sum_{f \in C  \setminus \{e\}} y_f \label{eq:circle}\\
%\forall e = (v,w) \in E_{\mathrm{lift}}^{\mathrm{time}}  \, \,  \forall P \in vw \textrm{-paths}(G_{f}) : y_e \leq \sum_{e' \in P} y_{e'} \label{eg:lift-path}\\
%\forall e = (v,w) \in E_{\mathrm{lift}}^{\mathrm{time}}  \, \, \forall C \in vw \textrm{-cuts}(G_{f}) : 1 - y_{e} \leq \sum_{e' \in C} (1-y_{e'}) \label{eg:lift-cuts}
%\end{multline*}
%\vspace{0.02in}
%\end{minipage}}
%\\
%where $y: E' \rightarrow \{0, 1\}$ is an edge label functions used to assign an edge $e \in E'$ belong to the same ($y_e = 0$) or distinct cluster ($y_e = 1$), the $\textrm{cycles}(G_{f})$ denotes for any circle in graph $G_f$, $vw \textrm{-paths}(G_{f})$ is any path in $G_f$ connecting $v$ and $w$, and $vw \textrm{-cuts}(G_{f})$ is any cut in $G_f$ assigning $v$ and $w$ to different groups. The first constraint guarantees that for any neighboring $v$ and $w$, if there exists a path from $v$ to $w$ in $G_f$ and along this path all nodes are labeled to $0$, then the edge $vw$ has to be $0$. The second and third constraints force that the label $y_{vw} = 0 \textrm{ with} \, (v,w) \in E_{\mathrm{lift}}^{\mathrm{time}}$ if and only if $v$ and $w$ are connected in smaller graph in $G_f$ by a path of edges labeled $0$.


% \myparagraph{Solver for Lifted Multicut for Tracking}
% Since our objective function is the NP-hard problem ~\citep{keuper2015lifted}, we resort to efficient heuristics. We first compute a preliminary partition with the greedy additive edge contraction algorithm, followed by an improvement step with the Kernighan\&Lin local search procedure ~\cite{keuper2015lifted}. The solver is presented in Appendix.

In summary, our formulation has the following advantages. First, we optimize intra-camera (temporal edges) and inter-camera (spatial edges) simultaneously. Additionally, long-range interactions are also incorporated through lifted-edges in $E'$.
This results in a solution informed by cues from all cameras at once.
Second, the optimal number of trajectories is determined during the optimization. Third, our nodes in the spatial-temporal graph are tracklets, resulting in decreased execution time as the hypothesis space is significantly reduced.

% Third, even though the lifted multicut problem is NP-hard, the heuristics we use are efficient and efficient heuristics that return high-quality solutions in practice~\cite{keuper2015lifted}.

%\scalebox{0.84}{
%\begin{minipage}{1.15\linewidth}
%\vspace{0.1in}
%\centering
%    \begin{algorithm}[H]
%        \SetAlgoLined
%        \DontPrintSemicolon
%        \KwInput{Graph $G_{f} = (V_f, E')$, affinity costs %$c_{e^{\mathrm{space}}},\, c_{e^{\mathrm{time}}}$
%        }
%        \KwOutput{Edge label function $y: E' \rightarrow \{0,\,1\}$
%        }
%        $y \leftarrow$ \textup{Greedy Additive Edge Contraction $(G_f, c_{e^{\mathrm{space}}}, c_{e^{\mathrm{time}}})$} \\
%        $y \leftarrow$  \textup{KernighanLin Algorithm  $(G_f, c_{e^{\mathrm{space}}}, c_{e^{\mathrm{time}}})$}\\
%        \textbf{return} $y$
%    \caption{Solver for Space-Time Lifted Multi-cut}
%    \label{alg:trans}
%    \end{algorithm}
% \end{minipage}}

 %------------------------------------------
% \subsection{Generating Tracking Predictions in 3D}
% \label{sec:3d-interpolation}
% Given clusters of the spatial-temporal tracking graph, we interpolate trajectories in 3D-coordinates.
% Since a cluster consists of a set of tracklets, which in turn consist of a set of detections, we directly associate a cluster with its underlying set of detections.
% Hence, let a cluster consisting of detections $\{b_1,\ldots,b_s\}$ be given.
% At each timestep $t$ such that there exists at least one detection in that timestep, we obtain a 3D position through
% \begin{equation}
% \begin{split}
% p_{avg}^t & = \frac{\sum_{i : \dettime(b_i) = t} h(b_i)}{\abs{\{i : \dettime(b_i) = t\}}} \\
% p_{3D}^t & = \argmax_{p : \norm{p - p_{avg}^{t}} \leq r } \sum_{i : \dettime(b_i) = t} \norm{\pi_{\cam(b_i)}(p), b_i}_{iou}^2
% \end{split}
% \label{eq:3d-interpolation}
% \end{equation}
% where $\pi_j(p)$ is the projection of a 3D cylinder centering at $p$ to a rectangle bounding box on 2D coordinates of camera $j$.
% The above interpolation step~\eqref{eq:3d-interpolation} first takes the average position of the 3D-projections of all relevant detections of a given timepoint.
% Second, a 3D position in the vicinity of the mean position is calculated such that the reprojection error w.r.t. IoU is minimized.


% %Given clustering results of the object $i^{th}$ at the time frame $t$, $\Gamma_{i,\,t} = \{b_{i,\,t}^{c_{1}},\, b_{i,\,t}^{c_{2}}, ...,\, b_{i,\,t}^{c_m}\}$, we estimate its 3D position by maximizing least squares problem:
% %\begin{equation*}
% %p_{3d}^{t*} = \argmax_{p_{3d} \in C = \{p: ||p-p_{\mathrm{avg}}|| \leq r \}} \sum_{j=1}^{m} w_{j}|| \pi_{j}(p_{3d}), b_{i,k}^{c_j}||_{{\textrm{iou}}}^{2}
% %\end{equation*}
% %where $\pi_j(.)$ is a projection that maps a cylinder centralized by $p_{3d}$ to view $j^{th},\, j \in (1, m)$. $||.||_{{\textrm{iou}}}$ is a iou score measuring overlapping given two bouding boxes, $w_j = 1$ if there exists a detection $b_{i,\,t}^{c_j}$ at the view $j^{th}$ and $w_j = 0$ otherwise, and $p_{\mathrm{avg}} = \sum_{j=1}^{m} w_j h(b_{i,\,t}^{c_j})/\sum_{j=1}^{n}w_j$, $r$ is a radius of circle centered at $p_{\mathrm{avg}}$. Optimizing the above least square problem 
%could also be considered as the post-processing step in case we are interested in 2D tracking results by projection the optimal estimated 3D cylinder into different camera views.

==> Lifted_Multicut _Optimization_for_Multi_Camera _Multi_People _Tracking/related-work.tex <==
\section{Related Work}
There has been a large body of research on single-camera MOT.
These methods focus on the data association step, for which the (lifted) multicut problem~\cite{tang2015subgraph,tang2016multi,tang2017multiple}, the lifted disjoint paths problem~\cite{hornakova2020lifted,hornakova2021making}, maximum clique~\cite{zamir2012gmcp,dehghan2015gmmcp},
multigraph-matching~\cite{hu2019dual}, and
binary quadratic optimization~\cite{Henschel_2018_CVPR_Workshops,henschel2016tracking,henschel2020simultaneous,von2018recovering} was used.
Another area is building end-to-end differentiable frameworks for both detector and data association~\citep{wojke2017simple,chu2019famnet,bergmann2019tracking,zhou2020tracking,zhang2021fairmot}.
For an exhaustive survey of MOT we refer to \cite{dendorfer2021motchallenge}.

Multi-camera MOT has recently received increasing attention. The related work can be categorized into two different approaches: 
% \myparagraph{Single Camera MOT}
% The task of tracking multiple objects observed by a single camera has received ample attention and great progress has been made on standard benchmark datasets such as the MOTchallenge~\cite{MOTChallenge2015,MOT16,dendorfer2020tracking}.
% The state of the art approaches
% \cite{bergmann2019tracking}
% and
% \cite{zhou2020tracking}
% rely on powerful object detectors but employ only greedy or frame-to-frame data association, thus are prone to ID-switches and suffer when long-term occlusions are present. In order to improve upon similar simple data association procedures, several optimization formulations have been employed, among them
% the (lifted) multicut problem~\cite{tang2015subgraph,tang2016multi,tang2017multiple},
% %
% the lifted disjoint paths problem~\cite{hornakova2020lifted},
% %
% maximum clique~\cite{zamir2012gmcp,dehghan2015gmmcp},
% %
% maximum independent set~\cite{brendel2011multiobject},
% %
% multigraph-matching~\cite{hu2019dual} and
% %
% binary quadratic optimization~\cite{Henschel_2018_CVPR_Workshops,henschel2016tracking,henschel2020simultaneous,von2018recovering}. Taking into account the data association while training the corresponding costs has been proposed in
% \cite{braso2020learning}. In general, single camera trackers are very powerful and are based on sophisticated re-identification features.
% Hence, it makes sense to use their power in the multi-camera setting as well.
% \begin{table}[!hbt]
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{cccccc}
% \Xhline{2\arrayrulewidth}
% Method & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Single-Camera\\ Tracklets\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Centralized \\ Representation\end{tabular}} & Online \\ \Xhline{2\arrayrulewidth} 
%     \small {LMGP (Ours)} & \checkmark & \checkmark & \\
%     \small{MLMRF} \cite{lan2020semi} &\checkmark & &\checkmark \\ 
%     \small{TRACTA}\cite{he2020multi} & \checkmark &\\
%     \small{DMCT} \cite{you2020real} & & \checkmark & \checkmark \\
%     \small{GLMB} \cite{9242263} &  & \checkmark & \checkmark \\         \Xhline{2\arrayrulewidth}
%     \end{tabular}}
%     \vspace{0.05in}
%     \caption{
%     Comparison of our LMGP w.r.t.\ recent multi-camera trackers.
%     Single camera tracklets signifies for trackers whose inputs can be used as tracklets. Centralized representation refers to usage of relationships among detections at each timeframe. Online indicates for only current frames are used. 
%     }
%     \label{table:reference-compare}
%     \vspace{-0.2in}
% \end{table}

\myparagraph{Single View-Based Methods} 
\cite{xu2016multi} propose a Hierarchical Composition of Tracklet (HCT) framework to match local tracklets by utilizing multiple cues of objects such as appearances and their 3D positions. 
% \citet{bredereck2012data} employ a Greedy Matching Association (GMA) method, which iteratively pairs local tracklets obtained from distinct cameras one by one. 
In \cite{xu2017cross} the matching problem is solved using a Bayesian formulation with a Spatio-Temporal Parsing (STP)-based tracking graph to prune matching candidates by exploiting semantic attribute targets.
Similarly,~\cite{wen2017multi} formulate a dense sub-hypergraph search (SVTH) on the space-time-view graph using a sampling-based approach.
Recent approaches include a semi-online Multi-Label Markov Random Field (MLMRF) method~\cite{lan2020semi}, where the ensuing optimization problem over single detections is solved through alpha-expansion~\cite{boykov2001fast} and a non-negative matrix factorization approach (TRACTA) for grouping tracklets across cameras~\cite{he2020multi}.
In another direction, DyGLIP~\cite{quach2021dyglip} formulates the data association problem for multi-camera as a link prediction on a graph whose nodes are tracklets. 
While these methods have demonstrated promising performance in some datasets, they are affected by ID-switch errors in the tracklet proposal generation, especially in cluttered or crowded scenes such as~\cite{chavdarova2018wildtrack}.

\myparagraph{Centralized Representation-Based Methods} To estimate the occupancy map (2D) or occupancy volume (3D), occlusion relationships among different detections have been explicitly modeled. The works in ~\cite{focken2002towards,mittal2002amulti} construct occupancy maps by using the foreground map after a background subtraction step.
Ground plane homographs are another technique introduced in \cite{khan2006multiview}, that generates a voting map from the foreground pixels in each view for occupancy map construction. Toward the probabilistic approach ~\cite{fleuret2007multicamera}, GMLP~\cite{9242263} jointly uses CNNs and Conditional Random Fields to model explicitly an occupancy volume map given detections estimated from multiple cameras. More recently~\cite{you2020real} (DMCT) propose deep learning to directly compute the occupancy volume by fusing feature maps extracted from CNNs at multi-camera views.

%  The methods in \citep{leal2012branch,hofmann2013hypergraphs} also extend  min-cost flow tracking to reconstruct occupancy map, but cannot model higher-order consistencies.

% \roberto{Several approaches extend  min-cost flow tracking to globally solve the multi-camera setup \cite{leal2012branch,hofmann2013hypergraphs}, but cannot model higher-order consistencies.}

% \myparagraph{Multi-Camera MOT}
% Relatively less attention has been paid to multi-camera MOT.
% Classical approaches extending the disjoint paths formulation previously used for MOT are~\cite{hofmann2013hypergraphs,leal2012branch}.
% Recent approaches include a semi-online MRF-based approach~\cite{lan2020semi}, where the ensuing optimization problem is solved through alpha-expansion~\cite{boykov2001fast},
% a hierarchical composition based approach~\cite{xu2016multi} incorporating multiple cues (ground occupancy consistency, appearance similarity, motion coherence),
% and a non-negative matrix factorization approach for grouping tracklets across camera together~\cite{he2020multi}.
% Semantic information such as actions of people in videos and face direction have been used in~\cite{xu2017cross}.
% An online tracker built in a deep network for estimating 3D ground points and person detections has been presented in~\cite{you2020real}.
% Explicit occlusion filtering has been explored in conjunction with a Bayesian filter in~\cite{9242263} and in a joint CNN+CRF model in~\cite{baque2017deep}.

\myparagraph{Differences w.r.t.\ Previous Work}
% Our work, denoted as LMGP, is inspired by single-view-based methods, with tracklets proposals generated from the single-camera CenterTrack \citep{zhou2020tracking}; however, we take advantages of centralized representation ideas to overcome ID-switch problems in previous studies through a novel 3D geometry-based occupancy map. This factor sets us apart from competing approaches. (more detail in Table 1, Appendix). Moreover, we are also the first to formulate a global lifted multi-cut method for multi-camera settings, which so far has only appeared for the single-camera method.
Our work, denoted as LMGP, is at the intersection of single-view-based and centralized representation methods. We use single-camera tracklets but improve them by eliminating ID-switch errors using centralized representation concepts with multi-camera information derived from a novel 3D geometry-based occupancy map.
This factor sets us apart from competing approaches (Table \ref{table:reference-compare} Appendix). Moreover, we are the first to formulate a global lifted multicut method for multi-camera settings.
So far, lifted multicut was only applied to the single-camera setting~\cite{tang2015subgraph,tang2016multi,tang2017multiple}. We argue that our model is an elegant abstraction capturing the full range of interactions in multi-camera MOT.

% Our work uses state of the art single camera trackers and combines them with 3D-reasoning and a global optimization model that jointly considers association between cameras and long-range temporal interactions. 
% This sets it apart from competing approaches as depicted in  Table~\ref{table:related-work-comparison}.


==> discussion.tex <==
\section{Discussion}
Besides a novel spatial-temporal lifted multi-cut formulation, our essential contribution is the 3D-based pre-clustering; thereby, we could address both perturbations in tracking graphs and composing high-quality affinity costs. Due to the 3D constraints assumption, this clustering step will depend on how calibrated camera parameters and bounding boxes are correct. While the camera parameters are simple to control, the bounding boxes are much more challenging as they are influenced by detectors and camera poses.  In our experiments, WILDTRACK satisfies these requirements, while in PETS-09, the bounding boxes are inferior due to the camera's position, and the DPM detector was employed. Consequently, we could achieve state-of-the-art performance on WILDTRACK with a large margin while much lower in PETS-09. In short, this phenomenon gives an insight idea that our method is highly suitable to track over a medium space given good detectors with multi-camera. We thus consider the obstacles to track in a vast space as challenges for future works. 
% For instance, if the camera positions are too far away targets tracking , even a state-of-the-art detector may suffer with small and error bounding boxes. Similarly, if the camera pose is close enough to pedestrian objects, low quality bounding boxes by a detector still may occur.

==> issues.tex <==
- multi-cut -> multicut (Done!)
- Change much more -> more, remove very unless really needed. In general, do not use superlatives. (Done!)
- In specific -> either Specifically or In particular (Done!)
- Consistent paragraph titles (Capitalization, punctuation) (Done)
- Use tenses consistently (do not switch without reason from present to past and vice versa). (Done)

- Have one big document and use proper references for stuff in the appendix. (Done)

- Update reference given a merge of the main and appendix file.  (Done)

